Optimization of GNN Training Through Half-precision

Recent trends in lower precision, e.g. half-precision floating point, training have shown improved system performance and reduced memory usage for Deep Learning while maintaining accuracy. However, current GNN systems cannot achieve such goals for GNN, as our analyses show that they massively underperform while showing abnormal accuracy when using half-precision. These systems suffer from value overflow issues due to lowered precision, under-utilization of hardware resources, and poor training performance. To mitigate this, we introduce HalfGNN, a half-precision based GNN system. HalfGNN proposes novel techniques: new vector operations for half-precision data types that improve data load and reduction performance, and discretized SpMM that overcomes the value overflow and natively provides workload balancing. Such techniques improve hardware utilization, reduce memory usage, and remove atomic writes. Evaluations show that HalfGNN achieves on average of 2.30X speedup in training time over DGL (float-based) for GAT, GCN, and GIN respectively while achieving similar accuracy, and saving 2.67X memory.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> tex/arch.tex <==
\section{Improving Kernel Designs}

%Almost all the steps are identical for these two sparse kernels (SpMM and SDDMM) with minor differences. 
%only difference in implementation is considering edge weights for SpMMve. Among different works of SpMM, 
%This allows for identical optimization opportunities.
%For our discussion, we will discuss common optimizations once.
%Some of the similar tasks performed for all 3 kernels involved are, loading NZEs(edge tensors) and vertex level tensors(feature matrix). For SpMMve we also need the edge weights. But this is done in the same step as edge level tensor loading. 
%During SpMMv the weights are 1, and for SpMMve, weights get their respective values. 
%There is some difference between SpMM variants and SDDMM. The minor difference with SpMM is that SDDMM needs to fetch vertex features of the row and column IDs of each NZE, while SpMM only needs features of column IDs. 
%Both of them are distributed among threads and reduction for dot product calculation follows.
%Another important thing to note is that data loading time is much more costly than actual parallel computation. This is a classic bottleneck situation, computation capability has reached far higher potential than loading and writing memory locations. So, it is often the case that how fast can we load the memory to the blocks, dictates a large portion of the performance. Careful implementations are required to minimize loading and writing time.


2 well-known paradigms, vertex-parallel, and edge-parallel are often how kernels are designed. In this section, we pick one edge-parallel system and one vertex-parallel system and show how to adapt various techniques proposed in this paper to the current state-of-the-art. 
We now present an edge-parallel and a vertex-parallel SpMM and SDDMM design on how to incorporate our proposed techniques.

\subsection{Edge-Parallel Kernel Design} 

In this section, we pick {\gnnone} design. It is currently the edge-parallel state-of-the-art system. {\halfgnn} fundamentally is an edge-parallel design also.

\subsubsection{\textbf{Edge-Parallel SpMM}}
GNNOne has three stages. We use those stages individually to describe what changes are needed. 

% Each warp handles XX NZE count. They perform and running sum of 


% \textbf{Vectorized SpMMv\/SpMMve} This combines all the aforementioned optimizations to get accumulations of reduction over all declared kernel blocks. This is the possible carryout for gather operation of a particular node, which has it's gather reduction computation split among blocks in an asynchronous way. This step is highly optimized, as it doubles the possible hardware utilization, thread throughput, dataloading \& reduction in atomic writes.\\
    
% \textbf{Handling Carryout} We can calculate the each node carryout of each block even before the carryout kernels are launched. This takes linear time and only done once before kernel launch. So, another kernel simply gathers reductions for each node distributed over blocks. This can be easily done in parallel. These 2 steps barely takes any time. 

%\subsection{Stage-1 Data Load \& Handling Non-conflicting Warp Level Writes}
 %As we have discussed before. We used shared memory to lead edge information. Each edge would have source and destination. This is required for message passing operations performed in GNN. The same is done for edge-weights. But these needs to be organized in a special coalesced manner so that it facilitates our access pattern, and improved throughput. As can be seen in the \textbf{listing 1}, each warps writes are non-conflicting, as they are all handling different vertex positions in most cases. For all these conflicting cases, not race condition can occur and we simply used in place normal writes, rather than using costly atomic operations.\\



\noindent \textbf{Stage-1 Data Load to Cache.}
{\gnnone} uses GPU-shared memory to cache the non-zero elements and edge features. Data load is distributed among warps equally. Each warp handles fixed-sized non-zero elements and their edge features.
%Each warp of 32 threads gets to load 128 edges in coalesced manner in to the shared memory. 
Caching in shared memory has been well-studied as the stored data can be reused for the rest of the computation.

{\halfgnn} continues to use caching, and still fetches in the same manner. However, for edge features, we rely on a half2 data type that effectively leads to faster loads. For features, {\halfgnn} still allows warps to fetch a fully coalesced memory access, but in our case, we employ vectored data load to reduce effective memory barriers, \& latency to extend hardware utilization.
%However, we propose a simple change here: as the 2 edge features are loaded by each thread, their individual half are extracted and converted to half2 by mirroring the half values. 

\noindent \textbf{Stage-2 Data Load and Dot Product.}
In this stage, for {\gnnone}, each thread reads the same non-zero edge feature (one at a time) cached in shared memory,  fetches its different vertex features 
%in a feature-parallel way
(1 per thread), and performs a multiplication.

{\halfgnn} performs these same steps differently, that the threads now have vertex features and edge-features in half2, and hence a single multiplication product stage produces two dot products. 
%Shared memory being magnitudes faster than GPU memory, it helps greatly to improve performance. 

\noindent \textbf{Stage-3 Reduction and Write.}
GNNOne uses a running sum (reduction) till a row split is observed. Upon observing a row-split, it uses atomic instruction to write the dot product. At the end of handling 128 NZEs, each warp also atomically writes the last reduced values. 

{\halfgnn} continue to use half2 and does perform running sum using half2 intrinsic. However, the big difference is that we do not perform atomic write at all. As our \emph{non-atomic design} shows we can make intra \& inter-CTA conflict resolutions for gathering and writing reduction of destination vertices, and use 2-stage kernels that get the job done with massive performance gain. 
%We first perform a inter-block reduction so that a row spread across warps within a block get a chance to reduce to generate a carry-out \td.

We are using an edge-parallel solution for \emph{SpMM}, and we are using our proposed \emph{Discretized Scaled SpMM}. This is because \emph{Discretized Scaled SpMM} allows complete training of GNN in \emph{half-precision}. Without it, no system can train GNN in\emph{half-precision}.

%We are distributing 512 edges total computation to 1 block. Rather than performing the normalization at the end (1) or in the beginning (2), we choose to perform normalization during each write inside the block in descritized manner (\emph{Discretized Scaled SpMM}). This can be thought of as computing the normalized reduction in a segmented manner per block, rather than doing it after the total reduction. This removes the vanishing gradient problem of (2), as our normalization would not decrease these values massively. Secondly, we are normalizing for reduction per block, rather than reduction per vertex at the end. So, the values should be within the range. This solution does not suffer from either of the problems of (1) or (2). 

%2 things are very important here, they are : to use shared memory and memory coalescing. 
%Hence, each block is allocated shared memory for 512 edges. This allows for the workload to be distributed among warps in coalesced manner, and most importantly helps our kernel implementation to reduce costly writes that would be otherwise unavoidable. %It will be discussed further in the kernel implementation section.

%Second thing is that each warp has a global positioning inherently among all the blocks and warps. As we distribute 128 edges worth of work in a load balanced manner, we do not need meta data or additional computation logic to access required memory locations for vertex level tensors. All that is required is to multiply the global warp-id with 128 (WARP\_EDGE\_BLOCK) and we can directly access the feature tensors. 
%In our computation we achieve double the memory access, double the computation that was previously possible. In the following section we will elucidate upon this.

% %\textbf{Homomorphic Type Conversion \& Vector Support}
% \textbf{Type Conversion \& Vector Support}
% As discussed before we bridge the research gap of GPU hardware support for half datatype, vector type and existing systems not increasing performance using them. In this section, we briefly overview a few key important steps for achieving this. Datasets for graph neural networks would  be in float32. Before passing it to kernels we simply convert these tensors in half precision(float16/16 bit floating point). This does not effect the performance of kernels in any significant manner. As we have discussed, earlier studies have shown that 16 bit in computations are enough for achieving great results, as long as the weights are stored in 32 bits. We want to follow the exact same approach for our work. This would allow only kernel implementations to be modified, but the rest of the things would be same for other works. So, we are targeting kernels that uses float16(half precision) datatype.
% Half precision alone does not improve the performance much. 
% %We combine vector arithmatic for threads to improve throughput. %This is due to the fact that just replacing float32 with float16 would not mean anything if we are doing the exact same computation. Exact same computation would lead to same number of cock cycles being used for kernel implementations. Although this improves memory requirement, it does not improve throughput. That is where the role of vector types come in.

% %Vector types are simple structures of basic types.
% In our work, we have extensively used pair of 2 half precision values (half2 datatype). For SpMMv, and SpMMve, we have to limit ourselves to only \textit{half2} datatypes. This is due to the fact that current GPU support only allows for \textit{half2} arithmetic and write operations. Though we can overload operators and create custom operators for various length of half types, this has one problem of atomic writes, which only supports at most \textit{half2} data type. Although we almost completely removed the need for atomic writes, it is still required for some cases, and using \textit{half2} reduces total required number of atomic writes by half. 





\subsubsection{\textbf{Edge-Parallel SDDMM}}

{\gnnone} has unified \emph{SDDDM} and \emph{SpMM} as both of them follow the same data-load design with the same stage-1 and stage-2 of data-load. The minor difference is that stage-1 does not load edge features, and stage-2 loads the vertex features of the row ID. However, in stage, it uses \emph{float4} data type to load the vertex features of row and column ID (source \& neighbor vertices) and performs a vector dot product to produce 4 dot products in each thread. The reduction stage is very different as the \emph{SDDMM} reduction happens across feature dimensions while \emph{SpMM} performs reduction across neighborhood dimensions. Hence, the reduction first does a thread-local reduction of 4 dot products to a single dot product before initiating an inter-thread communication. The final reduced value is written by a single thread to output tensor.
%Since reduction happens for each NZE that causes a memory barrier to be implied inter-thread communication

{\halfgnn} continue to use caching non zero elements in its stage-1 of data load, as we mentioned, it does not need to load edge features. 
In stage 2, we use \emph{float4} for kernel calls. But each float contains a \emph{half2} data type. For computation, we use \emph{half8} to load the vertex features of each non zero edge. That is, each thread loads 8 half features of row ID and column ID (source \& neighbor vertices) and performs their dot product using our \emph{vectored custom arithmetic operators} to produce eight half dot products in 1 arithmetic operation. {\gnnone} used to multiply 1 feature from source with 1 feature of neighbor. In {\halfgnn} we get 8 in 1 arithmetic operation. These 8 products are summed using half2. Finally, we use inter-thread communication to reduce the dot products produced by other warp threads. We require much fewer inter-thread CUDA API calls than {\gnnone} due to our vectored operation. This also lessens the waiting time for the communication barrier. This also results in better load performance compared to {\gnnone} SDMM. Finally, the reduced values are converted to half and are written to output without the need for any atomic instruction. Our evaluation shows we get on average $1.84 \times$ the speedup from original {\gnnone} SDDMM.

%For SDDMM we experimented with \textit{half4} (group of 4 half precision), \textit{float4} (group of 4 float32), and also \textit{half8} (group of 8 half precision). All provided significant performance gain over non vectorized kernel implementations.




\begin{figure}[t]
  \centering
  \includegraphics[scale= 0.25]{figures/spmm diagram.png} % Adjust width and height as needed
 % \caption{SpMM vectored computation in half precision over warp, block, grid }
  \label{fig-spmm}
\end{figure}



\begin{figure}[ht!]
  \centering  \includegraphics[width=0.50\textwidth,height=.3\textheight]{figures/sddmm vector.png} % Adjust width and height as needed
  \caption{Vector implementation of SDDMM for 64 features}
  \label{fig-sddmm-dot-product}
\end{figure}

\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.50\textwidth,height=.30\textheight]{figures/vector supwarp.png} % Adjust width and height as needed
  \caption{Vector warp reduction, with less overhead for thread communication (may be remove. Too long picture)}
  \label{exp-halfgnn-sddmm-reduction}
\end{figure}


% %previous.\\
% \label{sec.data-load}
% In our work we distributed load equally among each warps. Each warps handles 32 threads corresponding to 64 features (we used half2 as discussed before), over 128 edges. For dimensions like 128, 256 more blocks are declared where each threadIdx.x position would work on different feature ids. 


%\subsection{SDDMM}
%All the dataloading, and thread utilization optimizations apply for the SDDMM kernel. The workload distribution is similar for all the warps involved as before. This time graph $A$ provides the topology for which vertices are to be used for the dot product. Each thread is assigned 4 floating point structures. Each floating point contains 2 halves. As discussed before, we can easily switch types using simple pointers. So, float4 stands for structures of 8 half values grouped together. When 1 thread performs in-place multiplication, it takes 8 half-precision values from 1 vertex tensor, and 8 from another, and multiplies them. We get multitudes of throughput for this reason, as a single thread does many more computations per clock cycle. For some operations, we are getting as much as 8 times the per thread activity. Apart from that, we have to handle the reduction of multiplication of the feature vector of 2 vertices. We augmented the reduction kernel with vectorized computation that can take advantage of vector types. \\


%\red{reduced inter-thread communication}One of the key advantages of using \emph{half4, half8} is that during reduction, we need fewer inter-thread communication. This is possible because, with each thread communication, we are getting 4 communications for \emph{half4}, and 8 communications for \emph{half8}. As hardware support is only available for \emph{half2}, the last reduction has to be reduced using \emph{half2}. In the evaluation section, we showed the relative performance gain.

%One tricky thing was to switch between vector types so that we can use thread communication in CUDA. For vector types like \textit{float4},\textit{half4}, or \textit{half8} there are no thread communication that is possible directly.\\



\subsection{Vertex-Parallel Kernel Design}
We pick Huang et al ~\cite{huang2021understanding} for this category as it performs the best among other vertex-parallel \emph{SpMM}. It uses neighbor grouping to impart workload balancing, where neighbors of each vertex are grouped in the set of 32, thereby only the last neighbor group has less than 32 neighbors.


\subsubsection{Vertex-Parallel SpMM}
Huang et al ~\cite{huang2021understanding} dedicates one warp to handle one neighbor group of a row. The cache size (shared memory) is fixed at 32 for each warp. Hence, the computation by any warp only produces a partially reduced value. These partial reductions are then directly written to output using atomic write. 
To support half-precision, we exploit these observations.

We use half2 for the data load of features. 
Since a warp is responsible for handling just one neighbor group, %we implement the segmented norm on the neighbor group.
the neighbor grouping introduces conflicting writing within a CTA (consisting of multiple warps) as well as inter-CTA conflicts. This is similar to the above edge-parallel \emph{SpMM}, and hence the removal of atomic write is straight forward and similar. We simply store the reduction of each group in \emph{carry-out buffer}. This write is non-atomic as mentioned earlier. The destination vertices are pre-calculated anyway in Huang \emph{SpMM} design.  We just need to figure out how many \emph{carryouts} are stored by each vertex. This can be easily done using Huang's internal mechanism during  neighborhood distribution.  Our non-atomic design improves the vertex-parallel \emph{SpMM} performance by $1.24 \times$ on average.

\subsubsection{Vertex-Parallel SDDMM}
Huang et al ~\cite{huang2021understanding} does not provide \emph{SDDMM} implementation. Many prior GNN systems do not provide \emph{SDDMM} implementation, as it is needed only in attention-based GNN such as GAT, and not by GCN. However, {\gnnone} observes that \emph{SpMM} and \emph{SDDMM} can follow similar system design principles for optimization. So, our demonstration for Huang \emph{SpMM} is enough to demonstrate the generality of our proposed optimizations \& their effectiveness.\\

\red{\textbf{we did not implement vertex parallel SDDMM, so the following may not apply.}}

\red{Since \emph{SpMM} by Huang et al performed better than other vertex-parallel \emph{SpMM}, we implement SDDMM following their SpMM design. We also implement a float version as a reference to show how much half-precision SDDMM can perform compared to its float-based SDDMM.
For SDDMM, we use the neighbor grouping and caching of SpMM. For fetching vertex-features, we use float4 and half8 for float-based and half-based SDDMM. }







\begin{comment}
    


\begin{lstlisting}[language=c++, caption={\small{Kernel Pseudocode for SpMMV, SpMMVE variant}}, label={spmm_code}]
SpMM(COO graph, half* edge_weight16, half*  x16, half* y16, int total_dim) {
    __shared__ uint64_t s[N*BLOCK_EDGE_CHUNK];
    __shared__ edge[BLOCK_EDGE_CHUNK]
    // type conversion
    int id = threadIdx.x;
    int col_id = id + blockIdx.y * blockDim.x;
    int warp_id = threadIdx.y;

    int abs_warp_id = global_warp_id(warp_id);
    int warpStart = abs_warp_id * WARP_EDGE_CHUNK;
    int warpEnd = warpStart + WARP_EDGE_CHUNK;

    // half2 loads of edge_weights in edge
    // coalesced edges & edge_weight loading
    __syncwarp();

    edge_uni_t p1;
    int old_src;

    p1.comb = sh_dst[0];
    old_src = p1.edge.dst;

    half2 zero = __float2half2_rn(0.0f);
    half2 mySum = zero;
    for (int j = 0; j < WARP_EDGE_CHUNK; ++j) {
        p1.comb = sh_dst[j];
        
        edge_val = edge[j];

        if (old_src != p1.edge.dst) {
            half2y[old_src + col_id] = mySum;
            old_src = p1.edge.dst;
            mySum = zero;
        }

        mySum = __hfma2(edge_val, x[p1.edge.src + col_id], mySum);
    }

    // handle carryout in asynchronous fashion
}
\end{lstlisting}

But, this does not complete the implementation, a large part is dedicated to handling writes that are conflicting for each warps. Assume this condition, when a vertex have neighborhood information situated in both or multiple warps. This time, atomic writes are necessary. Warps are individual execution blocks, and computations are carried out in warp level by the GPU, so atomic writes can not be avoided.

\subsection{Stage-2 Handling Conflicting Warp Level Writes}
These carries can not only be distributed among warps in the same block, but also for larger feature sizes, carries can span across different blocks each having multiple warps. Each block in the execution configuration are assigned to different SMs, GPU scheduler carries out the distribution. And block to block communication is not possible. These carry out operations have to be atomic for this very reason. Required kernel implementations were designed to handle these atomic writes.
\end{comment}



%%%%%%%%%%%%%%%% old stuff %%%%%%%%%%%%

\begin{comment}

\noindent \textbf{Data Reuse.}
The loaded data is cached temporarily in the shared memory of the GPU so that it can be reused in stage 2.
For \textit{SDDMM}, the row ID and column ID of each NZE are needed in Stage 2 by multiple threads to fetch their vertex-features (vector), and their data-reuse is achieved by caching them in Stage 1.
However, the Edge-parallel SDDMM in prior works, such as DGL~\cite{dgl2019}, FeatGraph~\cite{featgraphsc20}, etc. do not have any caching strategy at all, and therefore cannot benefit from the data-reuse of NZEs.
 %Hence, we cache them during the stage 1 data-load in the shared memory of the GPU.

For \textit{SpMM}, NZEs are also reused:
the column ID of NZEs is reused by many threads to fetch their vertex-feature Stage 2, while the row ID is needed to reduce the dot products and write the result (vector) to output tensor.
Stage 1 additionally caches the corresponding edge-feature of every NZE which is needed by different threads to perform the dot product with the vertex-features. 
Therefore, The reuse factor for the cached elements in both SDDMM and SpMM is exactly as the feature dimension of vertex-features. 




\subsubsection{CACHE$\_$SIZE Determination and Discussion} \label{sec.cache_size}
%The separation data-load into two stages brings many novel opportunities for optimization that have not been explored by prior works, and many times are not possible in prior design.

The separate Stage 1 in {\name} allows us to find the cache size independent of row-length of sparse matrix or feature-length of each vertex, which is not the case in prior sparse kernel works, as we discuss soon. 

\noindent \textbf{CACHE$\_$SIZE and Memory Barrier.}
{\name} determines the cache size based on the hardware characteristic, such as thread count in a warp, shared memory size, etc., and not based on row-length of the dataset. %and based on support for special vector load instructions, such as float2/int2 or float4/int4 load instructions (\td not sure whether float2/int 2 is correct here). 
Hence, any multiple of 32 is a good starting point for $CACHE\_SIZE$. 
%even without using any vector load instruction.  However, one can also use vector load instruction to optimize it even further. 
Kindly note that a memory barrier is needed before Stage 2 can read the cached data from the shared memory. This incurs costs, specifically, memory-related instructions can not be reordered across a memory barrier. Hence, in the case of 32 as $CACHE\_SIZE$, each warp thread only issues one data-load, and then waits for the barrier.
%as not more than one data-load can be issued before the warp waits for the barrier.
%\red{That is because each thread in the warp can only issue one data-load and then need to wait for the barrier,  which incurs extra costs.}
However, by caching more than 32 elements, such as 128, the frequency of this barrier usage is reduced, allowing every warp thread to issue 4 data-load before waiting for the memory barrier. Hence, performance is better when Stage 1 caches 128 NZEs than just 32, which is confirmed empirically (\cref{sec.exp}).
%and thereby these costs are mitigated.
Our experiments show that caching 128 NZEs per warp brings better performance. 

%Clearly, separating the data-load phase into two stages {\name} can achieve a fully balanced data load and an optimal caching size in Stage 1. 


%Prior works, such as Ge-SpMM, GNNAdvisor~\cite{wang2021gnnadvisor} and Huang et al.~\cite{huang2021understanding} have cached 32 or smaller NZEs by any warp as they follow vertex-parallel variant, where caching is limited When the row-length. 
%is less than 32, they cache even less by a warp.
%Caching has been proposed by Ge-SpMM~\cite{gespmmsc2020} and is used by 


\noindent \textbf{Prior SDDMM Works.}
Sputnik~\cite{gale2020sparse}, FeatGraph~\cite{featgraphsc20}, dgNN~\cite{zhang2022understanding}, DGL, and others have not cached NZEs in their SDDMM.
Hence, they perform more data-load than necessary for loading NZE. Hence, Caching is very novel in SDDMM, and is enabled purely due to the similarity that we observe in this paper about sparse kernels.


\noindent \textbf{Prior SpMM Works and Row-Length.}
Vertex-parallel SpMM approaches uses a fixed cache size of 32, but also dependent on row-length. 
E.g., workload-balanced SpMM designs such as 
GNNAdvisor~\cite{wang2021gnnadvisor} and Huang et al.~\cite{huang2021understanding} break each row into neighbor groups of 32 non-zero columns, and are forced to use cache size to 32, unless it pre-processed with another neighbor grouping size. However, the last neighbor group and those rows that have less than 32 non-zero columns cache less than 32 NZE. 
GE-SpMM~\cite{gespmmsc2020}, caches only 32 NZEs. 
Even if such works do decide to increase the cache size, it is always limited by the row-length which varies for each row, as many rows that contain fewer non-zero columns are unable to fully utilize the increased cache size.
Hence, any vertex-parallel SpMM approach cannot make cache size independent of the actual computation. 
%\red{Hence, they always suffer from the impact of the memory barrier because such works can issue one data-load before encountering the barrier in the best case.}



\noindent \textbf{Prior SpMM works and Feature-Length.}
%The combination of caching NZEs (Stage 1) and thread-grouping (Stage 2) is unique to {\name}. has not been explored in prior SDDMM and vertex-parallel SpMM. even though some of the works have used float4 data-types internally.
Many SpMM works drop caching or have other behaviors when feature-length is less than 32, e.g., GE-SpMM drops caching. %This is because it allocates one warp to each row, and observes that it can only use 16 threads if there are 16 features for each NZE using the feature-parallel method. to load the feature of NZE,  The remaining 16 threads in the warp will be idle, which leads to low thread usage. 
On the other hand, GNNAdvisor, and Huang et al keep the warp threads idle while loading the features of NZEs. 
%Huang et al~\cite{huang2021understanding} does not support SpMM when the feature-length is less than 32. 
Since such feature dimensions are common, especially in the last layer of the GNN, a separate Stage 1 fully independent of Stage 2 holds significance and does not distinguish the implementation based on feature-length.

%The design of Stage 1 holds significance compared to the edge-parallel design in SpMV, where the latter does not require caching at all as the feature length is just 1, outlining the differences between SpMM and SpMV. (\td maybe remove it in future)

%Yang et al~\cite{yang2018design} is an edge-parallel SpMM work that extended the non-zero split of Merrill et al~\cite{merrill2016merge}. What about sputnik? \td



\subsection{Stage-2 Data Load \& Symbiotic Thread Scheduler} \label{sec.stage2}
%This stage is responsible for the data-load of vertex-features, and in addition, performs the dot products.
In SDDMM, this stage loads the vertex-features of row and column IDs of the cached NZE and performs their dot product. 
In SpMM, this stage loads vertex-features of the column ID of the cached NZEs, as edge-feature of NZEs are already loaded in Stage 1, and perform their dot product.

% As discussed in \cref{sec.overview}, each thread loads at least 4 vertex-features, i.e. one thread is mapped to at least 4 consecutive features by the Symbiotic thread scheduler.
% These dot products need to be reduced along different dimensions for SDDMM and SpMM. Hence, the scheduler decides which thread should load which feature(s) so as to maximize data-load performance by studying the impact of the memory barrier (due to inter-thread communication introduced by the reduction stage) on data-load amid better data-reuse as discussed next. 


% \noindent \textbf{Analysis: Impact of Memory Barrier on Data-Load.}
% For SDDMM, the reduction happens along the vertex-feature dimension for each NZE. 
% To illustrate, assume 32 as the feature-length. So, in the vanilla feature-parallel method, there are 32 dot products, each residing in individual threads of the warp. When using a tree reduction methods~\cite{featgraphsc20}, it requires \textit{five rounds of} inter-thread communication ($log_{2}^{32}$). 
% However, inter-thread communication either through shared memory or warp-level intrinsic (e.g., $shfl\_down\_sync$()) introduces a memory barrier.
% %To elaborate, the shared memory mechanism entails the invocation of an explicit memory barrier, while warp-level intrinsic brings an implicit memory barrier. 
% Unfortunately, memory barriers prevent the compiler’s optimization ability as it cannot reorder \textit{memory operations} (e.g. data load) across the barrier. This limits the instruction-level parallelism (ILP) for fetching features, leading to slower data-load performance.



\noindent \textbf{Thread-Group and Need of Scheduling.}
The symbiotic thread scheduler uses one thread to load at least 4 features so that the compiler can issue more data-load instructions before a memory barrier is hit. This leads to forming thread groups within a warp to utilize all its threads for various feature-lengths. E.g., if the feature-length is 32, then 8 threads are dedicated to loading them forming one thread group. Hence, there are a total of 4 thread groups within a warp. 
%Hence at any time, a warp processes 4 NZEs simultaneously in this feature-length case.
%Thread grouping is a logical primitive and depends on the feature-length as the latter is a run-time argument. 
%Hence thread groups also become dynamic. For instance, 
But in case 16 as feature-length, 4 threads form a thread group, resulting in 8 thread groups within a warp. 
%For feature-length 64, there are just 2 thread groups in a warp. 
Also, the count of NZEs processed simultaneously within a warp depends directly on the thread-group count within the warp. I.e., if the thread-group count is 4 (feature-length 32), each thread group handles one NZE, leading to 4 NZEs handled simultaneously by the warp. 
Further, the cached NZEs are divided equally among thread groups to process.  E.g., if the $CACHE\_SIZE$ is 128 then each thread-group is assigned 32 NZEs 128/4) to process independently.

This leads to \textit{two scheduling decisions to be made}: a) which 4 features are allocated to a thread (\cref{sec.feat_schedule}); and b) which NZEs are allocated to a thread group (\cref{sec.grp_schedule}).
As we explain next, such decisions present challenges on how to keep the coalesced memory access of the warp so that the data-load does not degrade.





%\noindent \textbf{Memory Coalescing through Scheduling.}
%Mapping one thread to four features is inspired by SDDMM reduction analysis to allow the compiler to issue four outstanding data-load instructions before observing the memory barrier. 

\subsubsection{Vertex-Level Feature Assignment Policy} \label{sec.feat_schedule}

Allowing a thread to issue four outstanding data-load instructions for feature loading may break the memory coalescing as the warp (or thread-group) cannot fetch consecutive 32 features (128 bytes) at one time even when the feature-length is 32. It requires careful design to allow memory coalescing.
%However, {\name} makes sure that this mapping does not degrade the memory coalescing while loading the features.
{\name} turns to a CUDA's native support for vector data-load instruction, such as \textit{float4}. This enables each thread to fetch 4 consecutive vertex features by using a single vector data-load instruction.
So, for 32 feature-length, a thread-group consisting of 8 threads achieves full coalesced memory access of 128 bytes. Moreover, it requires just 3 rounds of inter-thread communication ($log_2^8$) compared to the earlier 5 rounds.
%the proposed thread-grouping never degrades Stage 2 data-load performance. 
Results in \cref{sec.exp} shows that switching to the proposed thread-grouping leads to a significant speedup of %1.79$\times$ 
over the vanilla feature-parallel method for feature-length of 32.

%\noindent \textbf{Discussion.}
%We must carefully understand the source of this optimization. The usage of vector data-load ($float4$) instead of scalar data-load ($float$) is not directly responsible for the performance gain in SDDMM directly. 
%This is evident from the smaller speedup gained by SpMM using \textit{float4} data-type instead of \textit{float} data-type. 
%when we compare the performance of SDDMM when the feature-length is 128, where even the vanilla feature-parallel method fetches 4 features before the memory barrier. Hence, the performance improvement is usually less than \td \%. 
The huge speedup in SDDMM is because of performing more loads(each thread loads 4 features now) before the memory barrier, which leads to higher instruction-level parallelism (ILP) for data-load instructions. 
Hence, if one can come up with a different solution to increase ILP for data-load, it would provide similar optimization in SDDMM. However, not all solutions may perform better if they compromise with memory coalescing. E.g., an extreme design would be to dedicate a single thread to handle all vertex-features of an NZE to perform a full thread-local reduction. This will impact Stage 2 data-load performance warp cannot produce coalesced memory access. 
%as a single thread would be responsible for loading the vertex-features of an NZE, thereby their memory access pattern cannot coalesce within a warp.

%and due to fewer rounds of inter-thread communication. 
Since, using \textit{float4} easily provided the mechanism, we did not look for any other mechanism.
Though prior works have used vector data-load for various other purposes at different stages of sparse kernels, \textit{the unique proposal of {\name} remains novel in explaining the unknown impact that inter-thread communication creates on the data-load performance through the memory barrier.}

Though SpMM is different than SDDMM, thread-grouping is applicable to SpMM. So, each thread uses \textit{float4} data type during Stage 2 data-load. 
However, the usage of float4 does not bring significant speedup for SpMM because it does not perform inter-thread communication at the end of each NZE thereby observing no issues due to the memory barrier.



\subsubsection{NZE Assignment Policy} \label{sec.grp_schedule}
%At any time, each thread group works on a different NZE, therefore a warp fetches vertex-features of as many NZEs as the number of thread groups. To illustrate for the feature-length of 32 (i.e., 4 thread groups) and CACHE$\_$SIZE of 128 in Stage 1, each thread group is responsible for handling 32 NZEs (128/4). 
%that a warp is responsible for caching 128 NZEs in Stage 1, and
%However, which 32 NZEs should be assigned to each thread-group is the thread scheduling decision that we discuss in this sub-section.   
%This leads to another scheduling problem, which cached NZE should be assigned to each thread group within a warp.

We explore two thread-group scheduling strategies to decide which cached NZE should be assigned to each thread group within a warp. We explain these two strategies by using 4 thread-group (32 as feature-length), and 128 as CACHE$\_$SIZE.
%(strided and blocked) on how the thread groups are mapped to process NZEs, in which 
In the \textbf{Consecutive} method, the preferred method, the first thread-group is assigned the first 32 cached NZEs(0, 1, 2, ..., 31). The next thread-groups are assigned the next block of 32 NZEs, and so on. Each thread within the thread group handles different features of the same NZE. 
In the \textbf{Round-robin} method, the first thread-group gets NZEs stored in 0, 4, 8, 12, ..., 124$^{th}$ location in the cache. The second thread group gets NZEs stored in 1, 5, 9, 13, ..., 125$^{th}$ location in the cache, and so on.   
%assigns each thread-group 64 alternate NZEs. For instance, the first thread-group process NZEs stored in the 0, 2, 4, 6, ..., 126$^{th}$ location of the shared memory, while each thread within the thread-group handles different features of the same NZE. Similarly, the other thread-group handles all the odd NZEs in this case.
Listing~\ref{list-algo3} shows both methods of scheduling for thread groups of a warp.


% In the following section, we proposed a scheduling method to assign the thread-groups for the consecutive NZEs. This method is inspired by our analysis for SpMM since its reduction happens among the neighborhood dimension. However, the final scheduling policy leads to huge data-reuse in SDDMM and enables thread-local reduction, as well as better data-load performance in SpMM.


% \begin{lstlisting}[language=c++, caption= {gSpMMve kernel sketch for edge-parallel data load and dot product, when feature length (dim) is 32. We blidindly summed (reduced) all the dot products as we will correct it later when we dicuss actual reduction by row ID.}, label={list-load32}]
% void load_phase (int* nz, float* vtensor, float* etensor, int dim, int e_count) {
%   int t        = threadIdx.x;                                         
%   int lane     = t % 32;
%   int absWarpId= blockIdx.x*WARP_PER_BLOCK + t/32;
%   int eStart   = abs_warp_id* EDGE_CHUNK;                       
%   int eEnd     = eStart + EDGE_CHUNK;

%   for (int e = eStart + lane; e < eEnd; e += 32) {
%     sh_colId[id] = nz[e]; //Shared memory
%     sh_value[id] = etensor[e]; //Shared memory
%     __syncwarp();

%     for (int 0; i < 32; ++i) {
%       mySum += vtensor[sh_colId[i]*dim + lane]*sh_value[i];
%     }}}
% \end{lstlisting}

% So, if a row actually had 1000 neighbors, we can devise a solution that would allocate 1000 threads spread across thread-blocks, that can do this product independently. While for a vertex that only has 10 neighbors can just be allocated 10 threads. 


% int thdGrpId = lane / (dim/4);   
% int thdGrpLane = lane % (dim/4);   
% int thdGrpCount = 32 / (dim/4);

\begin{lstlisting}[language=c++, caption= {\small Sparse kernel sketch (simplified) for data-load Stage 2, showing thread-group scheduling.}, label={list-algo3}]
void SDDMM_or_SPMM_Stage2 (edge_t* coo, float* etensor, int dim, ...) {
  ... 
  //--Start of Stage 2
  //Calculate thread group details   
  int thdGrpCount = 4;//Example
  int thdsInThdGrp = 8; //Example
  int thdGrpId = warpLane / thdsInThdGrp;   
  int thdGrpLane = warpLane % thdsInThdGrp ;
  //EITHER Consecutive method
  int start = thdGrpId*CACHE_SIZE/thdGrpCount;
  int end = start + CACHE_SIZE/thdGrpCount;
  for (int i = start; i < end; i++){
    e = sh_edge[i]; //fetch the cached NZE
    ...
  }
  //OR Round-robin method
  for(int i=grpId; i<CACHE_SIZE; i+=thdGrpCount){
    e = sh_edge[i]; //fetch the cached NZE
    ...
  }
}
\end{lstlisting}

% \begin{lstlisting}[language=c++, caption= {\small Representative Partial Strided gSpMMve kernel Prototype: We only do a partial reduction and ignore the final reduction and write back to the output tensor. It assumes feature-length (dim) of size 32 or less}, label={list-algo-strided}]
% void SpMM_strided (edge_t* coo, float* vtensor, float* etensor, int dim) {
%   ...
%   //Stage2: Strided
%   float partialReduce[N];
%   int grp_id = lane / dim;   
%   int grp_lane = lane % dim;   
%   int grp_count = 32/dim; 
%   for(int i=grp_id; i<EDGE_CHUNK; i+=grp_count){
%     e = sh_edge[i];
%     if (e.rowId != oldRowId) {
%       partialReduce[pos++] = mySum;
%       mySum = 0;
%       oldRowId = e.rowId;
%     }
%     mySum+= vtensor[e.colId+grp_lane]*sh_value[i];
%   }
%   partialReduce[pos++] = mySum;
% }
% \end{lstlisting}



% \begin{lstlisting}[language=c++, caption= {\small Representative partial blocked gSpMMve kernel prototype: It shows blocked workload division within a warp when feature length (dim) is 32 or less. }, label={list-algo-blocked}]
% void SpMM_blocked (edge_t* coo, float* vtensor, float* etensor, int dim) {
%   ...
%   //Stage2: Blocked method
%   int grp_id = lane / dim;   
%   int grp_lane = lane % dim;   
%   int grp_count = 32/dim; 
%   int start = (32*grp_id)/grp_count;
%   int end = start + 32/grp_count;
%   float partialReduce[N];
%   for (int i = start; i < end; i++) {//Changed
%     e = sh_edge[i];
%     if (edge.rowId != oldRowId) {
%       partialReduce[pos++] = mySum;
%       mySum = 0;
%       oldRowId = edge.rowId;
%     }
%     mySum+= vtensor[e.colId+grp_lane]*sh_value[i];
%   }
%   partialReduce[pos++] = mySum;
% }
% \end{lstlisting}






%This method is even more useful when we cache 128 NZEs per warp, thread-local reduction can do more work, and minimize the number of items that need warp-level, CTA-level, and global reduction.

%of NZEs to a thread-group to load is not going to impact the coalescing opportunity. The feature-parallel technique still coalesces the loading of the features of one NZE.

We now investigate how reduction and data reuse influence the choice, and whether one can provide better data-load performance than the other.
%We now analyze two scheduling methodologies based on data-reuse and the amount of data exchange needed among thread-groups for reduction. 
%differs in how the reduction is performed, what their cost is for the reduction, and which method is better for the data load. These are discussed next.
%Yet, as we show later that blocked method performs better.


\noindent \textbf{Data-Reuse Analysis: Consecutive method is Better.}  
\textit{In SDDMM}, the Consecutive method introduces \textit{data-reuse of vertex-features of row ID} for many NZEs until a row split is encountered. This is because the COO is usually arranged in a CSR way~\cite{cusparse_coo}, and a block of consecutive NZEs is assigned to a thread group.
On the other hand, the Round-robin method offers very little data-reuse chance as consecutive NZEs are not allocated to the same thread group.
%and hence the vertex-features of the row will be reused unless a row-split is observed.
\textit{In SpMM}, no such data reuse exists irrespective of the scheduling method as vertex-features of a row ID are never fetched. 

%The consecutive method even offers a faster data-load than Round-robin method, as we show later in Fig.~\ref{exp-strided-blocked}. We explore the reason in \cref{sec.exp}.
%Hence, the final design turned out to be the blocked method for SpMM.

% It should be noted that the non-zero columns of a row may not necessarily have consecutive column IDs. Hence, none of the methods blocked or strided can coalesce more than feature-length of data access while loading vertex-features of the corresponding column ID. 
% Hence, in theory, none of the methods seems inferior to the other in this regard. 

% For the SpMM, no such data reuse exists. Hence, we need to realistically measure the stage 2 data-load performance. In order to do that, we forego reduction so that inter-thread communication does not influence the results. Hence, we rely on a partial prototype, where we rely on the running sum (reduction) of the dot-products without caring for its row ID. Yet, we need to make it realistic, specifically to handle the cases when the row splits during the processing of the cached NZEs. (\td add a example) This is because the two methods differ in how they observe the row split. To this end, the IF statements in the Listing simulate that case using the COO format. Stage 1 caches the row and column ID of each NZE.
%However, they differ in how data is reused and the shared memory is accessed. 






%than the SpMM counterpart: the cached NZEs, and vertex-features of the row.
%Though this seems a logical way of reusing the data-load, it has not been explored earlier. DGL does not keep the COO format in a CSR way, as it keeps CSR separately, and hence DGL cannot reuse the vertex-features of the rows. On the other hand, CSR-based SDDMM can introduce data reuse of vertex-feature of row ID but lacks workload balancing. Sputnik which relies on a custom storage format materializes the vertex-features of rows and columns, and reduced values to shared memory. This makes Sputnik very slow as we show in \cref{sec.exp}.




%\subsubsection{Dot Product and Reduction Analysis}
%For simplicity, we discuss the case when \textit{feature-length is just 32}, which is equal to the thread count in a warp.


%\noindent \textbf{SpMM.} (Listing~\ref{list-algo2}) shows that each warp thread picks the same NZE and loads its features using feature-parallel method, i.e.,  threads within a warp are now responsible for different feature dimensions of the same NZEs thereby achieving memory coalescing. During this stage, we also do edge-level computations, such as the dot product of vertex-features with edge-features.
%So, data loading along with edge-level computations use edge-parallel and feature-parallel both together.
%and does a dot product with the first stored edge feature. 
%This process is repeated for all the saved NZEs in a loop. Hence, the vertex features are loaded in fully coalesced way as well because feature length is 32. The dot product part does not need to use any atomic instructions and has no other thread dependency at all. Hence, data load and any edge-level computation are fully balanced irrespective of the row-length, as these two operations do not depend on the row ID yet. This step runs in a loop to handle all the cached NZEs and the corresponding edge features.

% However, reduction happens along the row, hence 
% The above design makes sure that we do not need to materialize the vertex-feature at all. 
% %Each thread only devotes one register while fetching the vertex-feature of the NZEs in feature-parallel way.
% However, we also want to make sure that we unnecessarily do not materialize all the dot products either in registers or shared memory. 
% This is because the total dot product in a warp for SpMM can be $EDGE\_CHUNK*feature$-$length$, which can be 4,096 dot products when $EDGE\_CHUNK$ is 128, feature-length as 32. Such a high count of the dot products will not allow high occupancy of GPUs; hence, the performance will suffer. Therefore, we also perform the running reduction with this phase. Thus, at any time, the partially reduced dot products are kept in the registers, consuming only one register per thread. This allows high GPU occupancy and also leaves us with the option of allocating more registers that we can devote to optimize Stage 2 even further, which we discuss later. \td. 

% \noindent \textbf{SDDMM.}
% %As {\name} is COO-based, Stage 1 loads and caches the row and column IDs as part of the NZEs in the shared memory. Hence, designing SDDMM becomes simpler.
% For each cached NZE, SDDMM fetches the vertex-features of the row and column both using feature-parallel method. 
% This is followed by doing a dot product of the features using the same feature-parallel method. Since the reduction in SDDMM happens along the feature dimension, hence an immediate reduction can be performed, and output written back. Hence, neither the vertex-features nor the dot products require any materialization. Clearly, SDDMM has no dependency on the row length at all. Hence, Stage 2 fully balances the SDDMM using feature-parallel load.

% %\noindent \textbf{Data Reuse Discussion.}
% Stage 2 introduces \textit{data reuse in vertex-features} for SDDMM.
% Since COO is arranged in a CSR way, the vertex-features of the row ID are reused for many NZEs until a row split is encountered in SDDMM. Thus, SDDMM introduces more data reuse than the SpMM counterpart: the cached NZEs, and vertex-features of the row.
% Though this seems a logical way of reusing the data-load, it has not been explored earlier. DGL does not keep the COO format in a CSR way, as it keeps CSR separately, and hence DGL cannot reuse the vertex-features of the rows. On the other hand, CSR-based SDDMM can introduce data reuse of vertex-feature of row ID but lacks workload balancing. Sputnik which relies on a custom storage format materializes the vertex-features of rows and columns, and reduced values to shared memory. This makes Sputnik very slow as we show in \cref{sec.exp}.



%Our analysis so far clearly favors the blocked method of thread scheduling. The next question that remains open is how the two methods perform for the reduction. This is an important question, as our aim is to optimize the data-load, but if the blocked method turned out to be inferior for reduction, we need to consider the trade-off between the performance of data-load (stage 2) and reduction.

\noindent \textbf{Reduction Analysis: Consecutive method is Better}.
%The reduction differs in SDDMM and SpMM. The former reduces along the feature dimension to generate output at the edge-level, while the latter reduces along the neighborhood dimension to generate output at the vertex-level. Hence SDDMM reduction has no role in deciding the scheduling method. So, we focus on SpMM reduction only.
\textit{In SpMM}, the Consecutive method is more useful for reduction as each thread group processes consecutive NZEs, which are likely to have the same row ID. Hence thread-local reduction can be performed along the neighborhood dimension by each thread-group. {Kindly, note the Consecutive method needs just one round of dot product exchange among thread-groups for the reduction in case two consecutive thread-groups have some NZEs of the same row ID.} 
%For example, considering there are only 2 thread-groups, and CACHE$\_$SIZE as 128, each thread-group needs to handle 64 NZEs. The blocked method only needs to exchange one set of dot products (equal to feature-length) in case both the thread-group handles the same row. 32 dot products (16 features * 2 thread-group * 1 NZE per thread-group). 
However, the Round-robin method requires more inter-thread communications for reductions as consecutive NZEs are assigned in a round-robin fashion to different thread groups. 
This is likely going to be more costly than a pure thread-local 
as this method needs to exchange 4096 items (32 features* 4 thread-group * 32 NZEs per thread-group) in the worst case. 
\textit{SDDMM} reduction has no role in deciding the scheduling method.


% To this end, the blocked method becomes more useful as each thread-group processes consecutive NZEs, and hence thread-local reduction can be performed. That is because many consecutive thread-group may be handling the same row, and thus only one round of inter-thread communication is needed. 
% \red{need to exchange 32 dot products (16 feature * 2 thread-group * 1 NZE per thread-group), as a row may span between the two thread-groups, i.e., 127$^{th}$ and 128$^{th}$ NZEs may be part of the same row.}

% However, the strided method requires many inter-thread communications for reductions as consecutive NZEs are assigned in round-robin fashion to different thread-groups. 
% This is likely going to be more costly than a pure thread-local reduction. 
%This is because consecutive NZEs are processed by different thread-groups. Hence, they always need to exchange the dot product among themselves as there is a high chance that the consecutive NZEs are part of the same row.
%as it tries to reduce only on alternate NZEs due to the strided method of workload division. 
%while each thread might have more than one item that requires intra-warp reduction.

% \red{To illustrate the severity of the problem that the strided method might generate for follow-up reduction, we calculate the total number of items in the warp that requires inter-thread communication for reduction. In the case of feature-length 16, it becomes 2048 items (16 features* 2 thread-group * 128 NZEs per thread-group) in the worst case.}
% %The worst case would have been observed when every NZEs are part of rows whose degree is less than 3. 
% %This case is when a warp caches just 32 NZEs. In reality, a warp caches 128 NZEs resulting in a much bigger count of items that require intra-warp reduction. 

It is clear that the Consecutive method is better than the Round-robin method. 
Moreover, a higher CACHE$\_$SIZE in Stage 1 favors the Consecutive method as each thread group handles more NZE, therefore it can do more thread-local reduction to minimize the thread communication in SpMM. Hence, the Consecutive method in Stage 2 is better suited to complement the Stage 1 design of caching more elements. 




% When fusion is desired, Stage 1 of the fused kernel fetches and caches both the NZEs and the corresponding edge-features. 
%where the former is used by both the SDDMM and SpMM while the latter is used only for SpMM.
% Thus, the fusion for Stage 1 is very natural without any additional complexities.
% Similarly Stage 2 fetches vertex-features of both the column ID and row ID, where the latter is used by SDDMM only. However, vertex-features of row ID are not fetched each time as they are reused, as discussed earlier.


% \red{
% \noindent \textbf{Unification Discussion}
% {\name} abstracts the computations for both SDDMM and SpMM into two components:
% 1. Efficient Feature Vector Retrieval which is optimal retrieval of the feature vectors associated with row and column IDs from each Non-Zero Element (NZE).
% 2. Coalesced Access to NZEs which involves the efficient and sequential read or write to each Non-Zero Element (NZE).
% By abstracting the computation in this manner, we enable unified reduction strategies and optimizations for both SDDMM and SpMM.
% }



%Besides that, this enhancement performs a 4(vertex-feature load of row of each NZE) + 4( vertex-feature load of column ID of each NZE) and their dot product before the memory barrier which enables the compiler to do the code optimizations.


%without sacrificing the coalesced access of NZEs and edge features. 

% each warp has 2 thread groups each with 16 threads. But there is only one thread-group per warp when the feature length is 32.
% Each thread group then works on a single NZE, while its individual thread works on its different features to achieve feature parallelism. 
% In the case of feature-length of 16, each warp handles 2 NZEs fetching 32 vertex features at one time in SIMT fashion, and the process repeats in a loop to handle all cached NZEs. 
% %Listing~\ref{list-algo2} (Step2) shows the high-level idea.

% The advantage of thread-group is that it is a logical concept and hence is very flexible, yet coalesces the data load of vertex-features. 
% Of course, when the feature-length is not a whole power of two, such as 6 in the case of the last GNN layer of  Citeseer, {\name} creates 5 thread-groups. Each thread group still 
% loads the vertex-features in a feature-parallel way to achieve the best under this circumstance by keeping only 2 threads idle in Stage 2. 
% % Of course, it never compromises on coalesced access of NZEs and edge features during stage 1.


% \noindent \textbf{Performing Dot Product.}
% During this stage, we also do some computations, such as the dot product of the vertex-features of the row and column of the non-zero columns in SDDMM.
% For SpMM, the computation becomes the dot product of vertex-features with the corresponding edge-features.
% %So, data loading along with edge-level computations use edge-parallel and feature-parallel both together.
% %and does a dot product with the first stored edge feature. 
% %This process is repeated for all the saved NZEs in a loop. Hence, the vertex features are loaded in a fully coalesced way as well because the feature-length is 32. 
% The dot product part does not need to use any atomic instructions and has no other thread dependency at all. Hence, data load and those computations are fully balanced irrespective of the row length, as these two operations do not depend on the row ID yet. 
% This step runs in a loop to handle all the cached NZEs (both SDDMM and SpMM) and the corresponding edge features(SpMM only).

%Caching a multiple of 32 NZEs, such as 128, is complex as Huang et al and GNNAdvisor need to change the pre-processing steps to make 128 a neighbor-group size. All the works need to introduce complex branching code to take care of multiple cases of their vertex-centric processing based on actual neighbor size, which may not necessarily be a multiple of 128. Branching introduces a slowdown in GPU.

% On the other hand, when the feature-length is less than 32, such as 16 which is of common use in original models of GCN, GAT, etc., prior works handle them differently. GE-SpMM does not use caching in this case, while GNNAdvisor and Huang et al. use a full warp, keeping many threads idle while fetching vertex features. We argue that these vertex-centric works cannot use caching without a full warp due to the memory barrier needed by caching, which can only be applied at the warp or CTA level.
% \textit{However, {\name} always caches 128 NZEs, and can vary this parameter without any significant changes.
% }

% In summary, caching and thread groups together achieve full coalescing for loading NZEs and edge features, while coalescing vertex features to the full extent. {\name} also avoids thread idling and reloading of NZEs and edge features.
%However, when the feature-length is not a perfect power of two, a few threads stay idle. For example, when the feature length is 6, such as in the output layer of GCN for Citeseer dataset, we only form 5 thread-groups each with 6 threads, leaving two threads of the warp idle during Step2.

%and hence they cannot achieve coalesced data load for all NZEs.  However, as discussed {\name} can cache more which leads to better performance. 

%Varying the number of cached elements is a simple exercise, as {\name} only requires the value of `EDGE$\_$CHUNK' to be changed. We show in \cref{sec.exp}, caching 128 elements improves the performance as it minimizes memory barrier usage, and is also beneficial in the reduction as we discuss in \cref{sec. coo}.

%Moreover, stage 1 is also independent of the length of the vertex-feature. This is in contrast to Ge-SpMM which does not do caching when the feature length is less than 32.
 
% If our solution has to be extended for gSpMV, we notice that caching the NZEs and edge features serves no purpose as they will be used just once. Once we drop the caching step, our SpMV implementation has to be either by Dalton et al~\cite{dalton2015optimizing} (or Bell et al) or Merrill et al~\cite{merrill2016merge} but using the COO format; though the COO format allows us to prototype both approaches together easily. 
% Hence, the paper does not generate any new insight for gSpMV. However, it remains to be answered whether the COO can perform better than or equal to CSR for these methods. 
% Since code by Merrill et al~\cite{merrill2016merge} is open-source, we do its variant, a pure non-zero split, using COO to compare against them to show that loading an additional 4 bytes for each NZE is better than the online search for row ID using pre-processed CSR.
%to prove that the COO has not been given equal opportunity. 
%We also evaluate the design trade-off using the COO format to explain the cost associated with materializing all the dot products.

\end{comment}



==> tex/challenge.tex <==

\section{Half-Precision GNN and Overflow} \label{sec.analysis}
%not converging at all for some larger datasets. 
%This is a problem, because for smaller datasets such as citeseer, pubmed, cora, it is of not much of realistic significance, as most datasets will be large, and only for large datasets we can really analyze performance achieved by applied parallelism. What these training results show that there must be some inherent problem in the implementations of half-precision implementation of DGL, for which we do not achieve the training results on par with 32 bits.\\
In this section, we investigate the reason behind overflow, and why some sparse kernels are never invoked in half-precision. That is, if half-precision based sparse kernels are being used at all, and if so what led to value overflow and whether the issues are due to GNN models or due to their system design and integration.
%limited range of half-precision as observed in \cref{sec.intro} where DGL training accuracy using half shows a higher accuracy degradation than float counterparts. 




%So, if we go over these limits, the result is either plus or minus INF which finally leads to $NaN$ due to later operations such as softmax operation that generates arithmetic using two INF. In this section, we discuss the two classes of GNN separately.


\subsection{\textbf{Actual Overflow}}
 
%Different from the issues discussed in the previous section, this sub-section shows actual cases of overflow which is not protected by mix-precision training. We talk about systems that do not break the SpMM into separate dot-product and reduction phases but design a single kernel to implement SpMM. 
%This class of GNN relies on \textit{unweighted SpMM}, such as GCN, GIN, etc. where edges contain no feature. Hence, this class does not suffer from the issues discussed \cref{sec.analysis.attention}. 
We observed that its SpMM kernel output values overflow on several mid-size datasets which shows that \textit{we have not designed Sparse kernels in the right way}. We find the root cause next on some popular GNN models, but discussions are general in nature.

\noindent \textbf{GCN.}
%, i.e., the edge features (the value of non-zero elements) are treated as 1.0. 
GCN uses unweighted {SpMM}, implying that each vertex directly aggregates features of neighboring vertices' features as the edge weights are absent or assumed to be 1.0. Our in-depth exploration shows that the aggregation in SpMM is responsible for overflow when a vertex has more neighbors irrespective of the system design of prior GNN systems. \textit{Overflow} condition implies that the value range is too small to hold the kernel output values, resulting in INF as output.   
%For smaller datasets such as Cora, Citeseer, and Pubmed, the neighborhood count is very small. 
Even modest-sized datasets such as Ogb-Product and Reddit, have many vertices with large enough neighborhoods. 
The INF values then produce NaN in the follow-up operations, such as softmax layer which involves operation using two INF.
%Our in-depth analysis shows that the problem originates during the SpMM operation for GNN, which first reports INF generation.

%The current GNN systems are not designed to handle this situation where our analysis has shown that SpMM computation first produces INF, and other kernels do not contribute to this. SpMM is performed in various ways for different GNN models, yielding different outcomes. With this in mind, we discuss two widely used GNN models to analyze whether these models have any mechanism to protect against overflow, and if so, how to take advantage of such mechanisms in system building.

%So, as datasets get larger, the chances are the gather operation will run into vertices, where gather crosses the range of half precision. This would have a catastrophic effect on the training. As such is shown in the experimental results shown in Fig. 1. 

We again question whether the overflow results from model design or whether any built-in mechanism exists to protect against the overflow.

Eq.~\ref{eq-gcn} shows a simplified computation involved in GCN.
where, \( \hat{\mathbf{D}} \) is the degree matrix of graph \( \hat{\mathbf{A}} \). \( \mathbf{H}^{(l)} \) is the activation of the previous layer, and \( \mathbf{W}^{(l)}\) is the weight matrix that is part of the linear layer. The linear layer transforms the activation of the previous layer, which then serves as input to the SpMM.
However, one can note the presence of the degree array in the equation where the degree array works closely with SpMM. The operation is called \textit{degree-norm}. GCN supports 3 different kinds of degree-norm: 1) degree-norm with the square root of in-degrees and out-degrees separately which is shown in Eq.~\ref{eq-gcn}; 2) degree-norm by in-degrees; and 3) degree-norm by out-degrees.


\begin{equation} \label{eq-gcn}
\large \mathbf{H}^{(l+1)} = \sigma \left( \hat{\mathbf{D}}^{-\frac{1}{2}} \hat{\mathbf{A}} \hat{\mathbf{D}}^{-\frac{1}{2}} (\mathbf{H}^{(l)} \mathbf{W}^{(l)}) \right)
\end{equation}


The degree-norm operator is present in GCN to add stability to feature values for training. To illustrate, consider the most used degree norm option 2 above, where the degree-norm operation is simply a division operator performed on the output of SpMM: divide the output features of every vertex produced by SpMM by its degree. A closer observation reveals that SpMM + degree-norm implies a `mean' reduction operation in SpMM, i.e. the aggregation stage in SpMM is mathematically equivalent to a `mean' operation. Hence theoretically it can never cause an overflow.   
%Most of the work has focused on option 1, which we analyze in detail, but the analysis is equally applicable to other options because the order of SpMM and degree norm is exactly the opposite in backward computation.

Clearly, the degree-norm operator is the built-in mechanism that can bring the SpMM output within the half-precision range. However, the current systems perform degree-norm division after the reduction (aggregation) in \emph{SpMM} is over, by then overflow has already happened.
Hence applying degree norms cannot help the values bring back within the half-precision range. 
A few prior GNN works have fused the degree-norm with {SpMM}. However, our analysis shows that such approaches are not helpful because they also divide the output of {SpMM} with the degree at the end of the aggregation, hence it cannot protect against overflow if we follow their approach in half-precision computation. 
%This problem arises in forward computation.


  
%The output of the SpMM can be thought of as producing vertex-level features, the degree-norm here divides each feature of vertices by the corresponding vertex degree. Hence, we focus on the output of a vertex for the combined operation of SpMM + degree norm operation, it becomes a ``mean'' operation on the features of its neighboring vertices' features.


%%%%//
%\td As we have discussed before, DGL provides 3 kinds of degree-norm. All of them are performed after the reduction operation is carried out for each corresponding vertex. We have presented that the reduction operation often overflows for some edges for 16 bits. The range is too small for half-precision reduction when it is not normalized. This happens as there are no changes for half-precision kernels, the sequence of steps being the same as it was for 32-bit kernels. This leads to large imprecision in computation, resulting in GNN not training well, and lowered accuracy results. 

%be able to normalize these accumulations and provide the stability that the authors of GCN proposed. 
%%%%//

\noindent 
\textbf{GIN.}
GIN has many variations, we focus on two variations. a) In the most common version there is no stabilization operation like the degree-norm discussed for GCN. This option is the default option in DGL, hence other works implement only this option. Therefore, there is no method to protect against the value overflow if one uses half-precision. 
b) DGL offers a few additional reduction operations in addition to the `sum' for the SpMM operation in GIN. One of those options is `mean' which is the same as SpMM followed by degree-norm as discussed in GCN. 
%reduction operation means dividing the \emph{SpMM} output by the degree, and hence this option is similar to the degree norm in GCN. 
%The other option that can be specified as a reduction operation in GIN SpMM is ``max''. By default, it cannot cause 
However, this option exists only in DGL and is implemented the same way as GCN, i.e., the degree-norm is called after \emph{SpMM} for forward computation. Consequently, this version of GIN is susceptible to the same overflow issue as GCN, while GIN implemented by other float-based GNN systems would always overflow. 

\begin{equation} \label{eq-gin}
h_u = \phi\left((1 + \epsilon) \cdot x_u + \sum_{v \in N_v} x_v\right)
\end{equation}

\blue{
Solving the overflow due to the reduction in SpMM is not sufficient as GIN also suffers from another overflow issue. Eq.~\ref{eq-gin} shows that GIN also scales up the source vertex features by $(1 + \epsilon)$, where $\epsilon$ is a learnable parameter. This part can also produce INF again, even if we take care of protecting the SpMM output from overflow.}





\textit{In summary}, unweighted SpMM computation is the root cause of the value overflow when using half for computation. GNN systems have a separate degree-norm which is equivalent to ``mean'' as a reduction operator which is a built-in mechanism to protect against overflow, but current GNN systems are not designed to take advantage of this. 
%Further, scaling the features of the source vertex in the GIN aggregation is another source of value overflow. 
%Other kernels do not contribute to value overflow.

%Otherwise, it causes the output generated by SpMM to go out of range when using half-precision. 
%There are a couple of solutions that can be proposed. However, the choice must be in line with kernel optimization for better performance in mind. Some of the design choices are as follows: 








%\subsubsection{Attention-based GNN models} \label{sec.analysis.attention}
%\subsubsection{Integration of Custom Kernel System to Mix-Precision}
\subsection{\textbf{Fear of Overflow}}
%We identify GNN models that can inherently handle the overflow, as class A. In GNN, SpMM is often accompanied by degree-norm. However, we observe that theoretically, it should be capable of preventing any overflow in half-precision, regardless of whether it produces overflow for most GNN models and all available systems. GAT is one exception among these. 
In this sub-section, 
%we focus on attention-based models, such as GAT, GaAn, AGNN, etc. Here, GNN models use weighted SpMM, where weight implies features on the edges. 
we show that \textit{integration of Custom Kernel System to Mix-Precision Training has not been clearly understood} thereby half-precision sparse kernels are not invoked as we explain next with a specific example of attention-based GNN, such as GAT,  followed by generalizing the observation.

\noindent \textbf{Exponential Operation in GNNs.}
%Hence, during the dot product stage, the vertex-level features of neighboring vertices are multiplied by the edge-level feature(s). This dot product stage is absent in the unweighted SpMM. We observe that scaling vertex-level features may prevent the value overflow in the follow-up reduction stage depending upon the mechanism to arrive at the value of the edge-level features.  
The final edge-level features in attention-based GNN, also called \textit{attention score ($\alpha_{ij}$)} as shown in Eq.~\ref{eq-gat}, are derived using an edge-softmax operator. This operator performs to find relative importance, where the exponential of $e_{ij}$ is normalized with the cumulative sum of the exponential of all neighboring attention coefficients. 
%But, it is not merely about the degree-norm, that prevents GAT from INF during half-precision, it is more so about how it is implemented. 
%Before this equation is computed, a series of {SDDMM} and SpMM variants give us 
Here, $e_{ij}$ are called attention coefficients which give importance of neighbor $j$'s feature to node $i$ are computed using other sparse kernels. 
However, DL frameworks such as PyTorch's mix-precision do not invoke half-precision computation of exponential operations as needed in Eq.~\ref{eq-gat}, 
but rather upgrade it to single-precision automatically. Thereby the attention score is never produced in half-precision. 
%An edge softmax operation is then 
%So the value range is always in (0, 1]. 
%while denominators are never 0 due to at least having self-edge. Hence, in this case, the weighted SpMM output of any vertex becomes a weighted average of the neighbor vertices' features. This provides inherent stability even for half-precision, and one does not need to alter SpMM to have similar accuracy. 

\begin{equation} \label{eq-gat}
\alpha_{ij} = \frac{\exp(e_{ij})}{\sum_{k \in \mathcal{N}_i} \exp(e_{ik})}.
\end{equation}

The exponential operation is immediately followed by an SDDMM variant to implement the division operation of Eq.~\ref{eq-gat} followed by an immediate SpMM.  
All these follow-up custom operations implemented by the custom back-end system receive float type tensor due to this upgrade of just one operation (exponential) to float type. 
%Hence, the underlying half-precision based kernels cannot be used at all, requiring either a full implementation of float-based kernels or performing an explicit data conversion of the tensors. 
%\textit{the custom back-end system receives a float-type tensor for its custom SpMM and SDDMM kernels} which immediately follows the exponential operation. 
%Hence, the custom back-end kernel remains unaware of the presence of mix-precision training and ends up invoking the float version of the sparse kernels.
This is an important observation, as exponential operation can produce value in the range (0, INF), hence PyTorch mix-precision stipulates that there is a real chance that half-precision is more likely to overflow when computing individual exponential. 
Thus, the GNN workflow has now been diverted from half-precision to float from the Custom Kernel System perspective. One is then forced to perform an explicit data conversion from float to half leading to code divergence, productivity, and maintenance issues.   


We question whether half-precision exponential operation leads to overflow or not in this specific case. 
Our studies for attention-based GNNs show that exponential operation cannot cause overflow because the model generates a negative number for attention coefficient ($e_{ij}$) as shown in Fig.~\td. Hence, its exponential is always in the range of (0, 1]. Therefore, the numeration of Eq.~\ref{eq-gat} can never overflow the half-precision. 
%Further, we show empirically (\td) that the denominator of Eq.~\ref{eq-gat} also cannot overflow the half-precision range.
% an equally important observation is that the GNN workflow now has diverted from half-precision to float from the Custom Kernel System perspective. One is then forced to perform an explicit data conversion from float to half leading to code divergence and productivity issues. 

\noindent \textbf{General Trend.}
Exponential is not the only operator where mix-precision automatically converts the incoming half-precision tensor to float before computing, but there are a range of operators that are used widely by multiple systems beyond attention-based GNNs that perform this upgrade. Specifically, the \td operations are used by Pytorch-Geometric~\cite{pytorchg2019} and MariusGNN~\cite{} to implement SpMM \td. Such operations are always performed in float even if the input is a half-precision tensor. Hence, such system designs cannot be migrated to half-precision computation. 



%These operations are performed with different variations of weighted SpMM. %Though, performance slowdown remains the major issue as was shown earlier in Fig.~\ref{fig-float-half-spmm} and \ref{fig-float-half-sddmmvv}.
%Thus, GAT is one such exception where a straightforward replacement of float with half-precision for SpMM would work without numeric issues for accuracy performance. 


%But, still, our system optimizations would be required to push the best available system performance, which we explore in later sections.

In summary, we observe that the fear of overflow has not allowed mix-precision training of the DL framework to offer a simple integration of half-precision custom sparse kernels to GNN training, leading to the invocation of float-based sparse kernels. This has serious implications on system designers as each Custom GNN System must implement both the float and half versions of sparse kernels and manually design a new GNN workflow based on the data type of tensors to perform the explicit data conversion. 



==> tex/exp2.tex <==
\begin{figure*}[h!]
  \centering
  \includegraphics[scale=0.45]{exp/exp-dgl-halfGNN-acc.pdf} % Adjust width and height as needed
  \caption{{\halfgnn} achieves the same accuracy as float DGL %\red{TODO: GAT fixed, Reddit Gin (error removed, NAN values now)}
  }
  \label{exp-dgl-halfGNN-acc}
\end{figure*}


%Hence, we evaluate several data science use-cases, as well as benchmark the graph preparation time.
\section{Evaluations} \label{sec.exp}

The following experiments aim to comprehensively evaluate the proposed optimizations and perform a comparative study compared to prior GNN works. All the experiments are conducted in NVIDIA A100 GPU which has 40GB of GPU memory. We conducted our experiments on 16 datasets mentioned in Table~\ref{table-dataset}. Only 5 datasets (Cora, Pubmed, Citeseer, Ogb-product \& Reddit) are labeled where accuracy is measured whose input feature lengths are shown.
Others are used for evaluating runtime only, hence they contain generated features.

This section focuses on GCN, GAT, and GIN models to show the overall effectiveness of {\halfgnn}. These models contain intermediate feature lengths of 64 \td (done). %respectively.
The intermediate feature length is important as the sparse kernels usually have this feature length during computation.

\begin{table}[t]
\small
\caption{Graph datasets. * denotes labeled dataset. F = Input feature-length, C = Prediction categories} % title of Table
\vspace{-6pt}
\centering % used for centering table
\begin{tabular}{l r r r r} % centered columns (4 columns)
    \hline\hline %inserts double horizontal lines
    Graph  & Vertex & Edge & F &  C \\
    Dataset & Count & Count &  & \\ [0.5ex] % inserts table
    %heading
    \hline % inserts a single horizontal line
    Cora (G1)* & 2,708 &  10,858 & 1,433 & 7\\ 
    Citeseer (G2)* & 3,327 & 9,104 & 3,703 & 6\\
%    ca-AstroPh & 18,772 &	198,110 \\
    PubMed (G3)* & 19,717 &  88,648 & 500 & 3\\
    % email-EuAll	& G3 & 265,214 &	420,045 \\
    Amazon (G4)  & 400,727 &  6,400,880 & 150 & 7\\ 
    Wiki-Talk (G5) & 2,394,385	& 10,042,820 & 150 & 7\\
    RoadNet-CA (G6) & 1,971,279&	11,066,420 & 150 & 7\\
    Web-BerkStand (G7) &685,230	& 15,201,173  & 150 &  7\\ 
    As-Skitter (G8)   &1,696,415 &	22,190,596 & 150 & 7\\    
    Cit-Patent (G9) & 3,774,768 & 33,037,894 & 150  & 7\\
    Sx-stackoverflow (G10) &2,601,977 &	95,806,532 & 150 & 7\\
   
    Kron-21 (G11) &2,097,152 & 67,108,864 & 150 & 7\\
    Hollywood09 (G12) &1,069,127 & 112,613,308 & 150 & 7\\
    % LANL & 31,142 & 115,949,436 \\
    % Kron-20 & 1,048,576 & 10,485,760\\
    Ogb-product (G13)* &2,449,029 & 123,718,280 & 100 & 47\\
    LiveJournal (G14) &4,847,571 &	137,987,546 & 150 & 7\\
    Reddit (G15)* &232,965 & 114,848,857 & 602 & 41\\
    Orkut (G16)  &3,072,627 & 234,370,166 & 150 & 7\\
    
%    Twitter & & \\
    % [1ex] % [1ex] adds vertical space
    \hline %inserts single line
\end{tabular}
\label{table-dataset} % is used to refer to this table in the text
\end{table}





% \begin{figure*}
%   \centering
% \includegraphics[width=0.97\textwidth,height=.11\textheight]{exp/exp-halfgnn-dgl-gcn-gat-gin-runtime.png} % Adjust width and height as needed
%   \caption{{\halfgnn}  vs DGL and {\gnnone}  Training runtime for feature size 64. It can be observed that the runtime of {\halfgnn} is much faster than DGL. We did not show the DGL half because  accuracy was not good as shown in figure ~\ref{obs-accuracy}, add good captioning and naming(\red{GNNOne k21 dim 64 not working})}
%   \label{exp-halfgnn-dgl-gcn-gat-gin-runtime}
% \end{figure*}


\begin{figure*}
  \centering
  \includegraphics[scale=0.45]{exp/exp-halfgnn-dgl-gcn-gat-gin-runtime-speedup.pdf} % Adjust width and height as needed
  \caption{{\halfgnn}  vs DGL, and {\gnnone}  training runtime speedup for feature size 64. (\red{DGL does not run for a few, GAT GNNone might have a bug.})}
  \label{exp-halfgnn-speedup}
\end{figure*}


\subsection{GNN Training}
This section evaluates the end-to-end training results, showing accuracy, runtime, and memory consumption.

\subsubsection{Training Accuracy} \label{sec.exp.accuracy}

%\begin{itemize}
%    \item GCN, GAT, GIN (pubmed, citeseer, cora, reddit, ogb-product)
    
%\end{itemize}

As we highlighted earlier in Fig.~\ref{obs-accuracy}, the accuracy of DGL for half-precision is much lower than the float-based models, which questioned whether half-precision is a viable option for GNN training.
%Hence, ~\ref{exp-dgl-halfGNN-acc}. This renders the possibility of systems such as DGL unusable, and more importantly incapable of getting any benefit that is available in half-precision training. For GCN and GIN, we can see that for smaller datasets DGL performs well for both half and full precision. But for GIN, DGL provides poor accuracy for half-precision in some cases. Only for GAT, DGL performs well both for half and full precision. This inconsistency of half-precision training for DGL is what makes {\halfgnn} very important(\red{TODO: fix GAT inconsistancy}). We can establish that the best accuracies for DGL are achieved in full-precision. 
Hence, we use DGL single-precision as the baseline in Fig.~\ref{exp-dgl-halfGNN-acc} to show that {\halfgnn} accuracy achieves similar accuracy to the baseline. \textit{This implies that half-precision is a viable option in place of float without compromising the GNN accuracy}. 
%For GCN, we can observe that for half-precision the accuracies are comparable to full-precision accuracy for DGL, and achieve the best possible accuracy across all the datasets. There was no drop in accuracy for {\halfgnn} (DGL half-precision showed a large drop).{\halfgnn} performs similarly for GIN, achieving the best possible accuracy for all datasets(\red {reddit not running in {\halfgnn} GIN}). This is in stark contrast to DGL half-precision, which failed to reach even $50\%$ accuracy during testing for some datasets. 
%Then we take a look at GAT, and the pattern is the same, with no drop inaccuracies. So, {\halfgnn} as a system achieves full accuracy performance using half-precision only. This makes the {\halfgnn} the only half-precision-based system for GNN to achieve such feats.\red{where to put the DGL half to show it does not work?}
{\halfgnn} achieves state-of-the-art accuracy for all datasets across GCN, GAT \& GIN. 
The reason for the same accuracy in {\halfgnn} as float-based DGL is identifying and protecting the overflow through the proposed \emph{Discretized} \emph{Scaled} \emph{SpMM} \& \emph{Scaled} \emph{Feature} \emph{Aggregation} 
\td (done) technique. Protection for \emph{SpMM} is possible only at the sparse kernel level as frameworks themselves cannot protect against such overflow. Furthermore, 2nd technique allows us to train for models that apply similar aggregation as GIN.

\subsubsection{Training Runtime} \label{sec.exp.runtime}
%\red{remove DGL half runtime talk, we will not include it}\\

%For this section, let us focus on figure ~\ref{exp-halfgnn-dgl-gcn-gat-gin-runtime}. 
Fig.~\ref{exp-halfgnn-speedup} shows the runtime speedup of training time of GCN, GAT, and GIN using {\halfgnn} over DGL and {\gnnone}. All the GNNs were trained for the same epoch(400) count. 
%Observing both of the full precision runtimes of DGL \& {\gnnone} would give us a good baseline to observe the characteristics of half2 vectored implementation. 
For the smaller graphs (G1 -- G3), prior work[\td no bibtex ] has shown that the training runtime is determined by the framework overhead and not by the GPU kernel runtime, hence we plotted only for larger graphs. The results show that {\halfgnn} achieves \td (done) $2.11 \times$ speedup over float-based DGL. Kindly recall that Fig.~\ref{fig-float-half-spmm} and Fig.~\ref{fig-float-half-sddmmvv} have shown that half-precision based DGL kernels are slower than float-based DGL. Hence, we picked the faster baseline here. 
{\halfgnn} also achieves \td (done) $1.24 \times$ speedup over {\gnnone}, which is the current state-of-the-art float-based system. 

%Among GCN, GAT \& GIN, {\halfgnn} provides the best improvements (in magnitudes of a couple of times for some datasets) for GAT training. This is because GAT involves kernels that can take maximum advantage of optimizations proposed in {\halfgnn}. This will be explored in further sections (todo). This experiment establishes the merit of integration of vectored half implementations of kernels into the {\halfgnn} system in terms of runtime. 
Compared to DGL float {\halfgnn} achieves $ 1.74 \times, 2.94 \times \&\ 1.64 \times$ speedup on average for GCN, GAT \& GIN respectively (\red{few does not run for DGL}). Compared to {\gnnone}, we get $1.22 \times, 1.13 \times$, \& $1.38 \times$ speedup on average for GCN, GAT, and GIN.

Thus, the results so far show that half-based GNN is not only feasible(\cref{sec.exp.accuracy}) but is also significantly faster to train.
The reason for the faster training time is the better sparse kernels of {\halfgnn} compared to prior GNN works, specifically introducing half-precision specific performance optimization to the sparse kernels of SpMMv, SpMMve, and SDDMM in {\halfgnn}. We show the runtime comparison of these kernels next by focusing on evaluating the impact of the proposed optimizations of {\halfgnn}.

%\begin{figure*}
%  \centering
  %\includegraphics[width=0.99\textwidth,height=.12\textheight]{figures/spmmv cusparse vs half2carryout PNG.png} % Adjust width and height as needed
  %\caption{CuSparse vs Half2 Carryout runtime for SpMMv. Todo: update for a17,a18,a19, \red{shift to speedups, no spmmv in cusparse}}
  %\label{exp-cusparsevsHalfGNN-spmm}
%\end{figure*}

%\textbf{Doubling Throughput at Warp\-level Granularity} 
%So, considering the runtime of {\halfgnn}, {\gnnone} \& DGL, it is obvious using half-precision, and equipping half with proposed optimizations for vectored implementations of SpMMv, SpMMve, and SDDMM. We can achieve much faster runtime compared to {\gnnone}, and DGL. 


%The next focus is on comparing with the standard DGL system.\\
%(mostly used, and industry standard state of the art).\\

%As in the previous sections, we foreshadowed how {\halfgnn} and GNNOne full precision provide faster runtime than DGL, this section provides the experimental analysis represented in figre. 8 to establish that as an empirical fact. First, we want to observe the obvious, for each observable (large enough graph dataset providing enough computational opportunity to observe differences), it can be seen that DGL (half or full precision) takes much more time to train than {\halfgnn} even for feature size 32. For some datasets, the half implementation of DGL was slower than full precision DGL, rather than faster. From fig. 8, comparing with the {\halfgnn}, it can be seen that the fastest runtime for DGL considering all the datasets for feature size 32 is much slower than {\halfgnn} runtime in half-precision for both feature size 32, and 64. 



\begin{figure*}[h!]
  \centering
  \includegraphics[scale=0.45]{exp/exp-dgl-halfgnn-memory.pdf} % Adjust width and height as needed
  \caption{{\halfgnn} requires much less memory to train compared to DGL full precision. (On average 2.28 times less.) \red{discussion GNNOne }}
  \label{exp-dgl-halfgnn-memory}
\end{figure*}



\subsubsection{Memory Consumption}
%\red{collected halfGNN for dim 64(half \& full ) gcn, gat, gin(plot the data and write),collected DGL float dim 64}\\
%\end{itemize}



In this section, we want to focus on one of the most important contributions of the paper, which is huge memory reduction during runtime. Data was collected individually and without any interference. For all 16 datasets, we can observe memory savings in Fig.~\ref{exp-dgl-halfgnn-memory} compared to DGL. This is significant, as this means we are truly getting the best out of half-precision, as we previously mentioned using {\halfgnn} results in no accuracy loss, and faster runtime. Now, our work has achieved all of the accuracy, memory, and runtime without compromising any of them. This is often very hard to achieve, a very rare phenomenon overall. To summarize the observable visualization represented in figure ~\ref{exp-dgl-halfgnn-memory}, we achieve 2.28 times less memory usage on average in our work, than standard DGL (considering all 3 GNNs, over 16 datasets). 
%The results are even more pronounced for larger datasets represented from G4 to G16.
\\



Now let us explore why that happens. For our work, we followed the mixed precision training~\cite{micikevicius2017mixed}. The main ideas prescribed were as follows: keep the master copies in single precision, intermediate operations in half-precision for backward, and forward, and lastly all state tensors in half precision. {\halfgnn}'s optimized kernels perform all the in-between operations in half, and thus while Pytorch uses these instead of DGL's (half/float), every optimization carried out in this work for each kernel contributes to the improvement observable in the measurement of full runtime metrics, a fair reflection of what is to be expected, considering all that has been mentioned. \\
%Our improved half-precision kernels simply provided better performances compared to DGL's fastest(full-precision, rather than half). \\

The main summary is that all the micro improvements (kernel level granularity, in half precision) result in improvements in the macro scale (overall improvement in training metrics). This work also expands the improvements achieved by ~\cite{micikevicius2017mixed} for various DNN models, by adding GCN, GAT, and GIN to the list. DGL has failed to take advantage of this mixed precision opportunity (observable in previous sections, half does not work). In the following sections, we provide further measurements to showcase these improvements over DGLs fastest kernel implementations (float/single-precision).\\
%To briefly point out, for DGL: it was often the full-precision kernels that were the fastest rather than half-precision ones. \\



\subsection{Kernel Evaluation}
As we have shown in previous sections we provide reliable and faster GNN training. In this section, we want to focus on individual kernel performances compared to established DGL/Cusparse kernel performance and compare with our results.


\subsubsection{SpMM Runtime}
%Fig.~\ref{halfGNN_vs_DGL_spmmve} shows that {\halfgnn} achieves $4$ to $64$ times speedup over Cusparse SpMM (check the numbers, separate SpMMv, SpMMve)for half-precision.\\ 
DGL uses Cusparse for SpMMve. We analyze over 16 datasets (G4 to G16) to measure the runtime of such kernels for feature sizes 32 and 64. We compared our runtime against Cusparse half and also Cusparse float. Fig. ~\ref{halfGNN_vs_DGL_spmmve} shows the comparative speedup of our implementation. We can observe that for for all datasets the speedup is massive in scale compared to Cusparse half implementation. Furthermore, these speedups are consistent over feature sizes 32, and 64.
%(\red{Todo: some are too big for Cusparse half, run again}).
{\halfgnn} SpMMve achieves almost $64$ \red{(actually 70)} times faster runtime in some cases. Shifting our focus to single-precision, it can be seen that Cusparse \emph{float/single-precision} is faster than its half implementation. We can look at the speedup of our implementation compared to Cusparse \emph{float/single-precision}. {\halfgnn} achieves faster runtime overall. We get speedups from $2$ to $4$ times. \emph{SpMMv} shares the same design principles \& optimizations. These speedups are observed due to  introducing vectored arithmetic operations, better data loading to shared memory, non-atomic writes, and removing memory barrier. Removing atomic writes contributes largely to this performance gain. This faster \emph{SpMM} helps improving the training time for GCN, GAT and GIN. %In the later section, we clarify using experiments showing the role of \textit{half2} and removal of atomic adds contributing largely.



\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.4]{exp/exp-spmmve-halfgnn-cusparse-speedup.pdf} % Adjust width and height as needed
  \caption{ \small Speedup of {\halfgnn} SpMMve compared to Cusparse single-precision \& half-precision, ($\log_{2}$ scaling). {\halfgnn} achieves $2.55$ \& $25.52$ times faster runtime compared to Cusparse single \& half-precision on average. }
  \label{halfGNN_vs_DGL_spmmve}
\end{figure}



\subsubsection{SDDMM Runtime}

Moving on, we compared DGL \emph{SDDMM} half and float with {\halfgnn} implementation. The same observation applies that DGL \emph{half-precision} kernels individually do not provide any runtime advantage over their \emph{float/single-precision} counterparts. This could be attributed to the fact that just using half instead of float without taking advantage of possible optimization opportunities mentioned in this work, is impossible. Our vectored usage of \emph{half-precision} allows improved optimizations compared to previous works to improve the performance of the \emph{SDDMM} kernel. We achieve this by expanding the number of arithmetic operations performed per instruction, by introducing vectored grouping of half precision through the usage of \emph{half2}, \emph{half4}, and \emph{half8}, and reducing latency. The inherent flexibility of vectorized arithmetic that is applicable to \emph{SDDMM} kernel as previously mentioned allowed for this massive speedup. Just observing the speedups in Fig.~\ref{dgl-halfGNN-sddmmvv} we can see that we get speedups up to $12$ times, and for most getting over $6$ times the speedup compared the half \& float DGL \emph{SDDMM}. There are similar large-scale speedups that can be observed for feature size 32 and 64. We gain speedups averaging $7.42$ and $7.12$ times compared to DGL \emph{single} and \emph{half-precision}. Even the lowest speedup observed for G9 is over $2.5$ times.

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.4]{exp/exp-sddmmvv-halfgnn-cusparse-speedup.pdf} % Adjust width and height as needed
  \caption{\small Speedup of {\halfgnn} SDDMM compared to DGL single-precision \& half-precision ($\log_{2}$ scaling). {\halfgnn} achieves $7.42$ \& $7.12$ times faster runtime on average compared to DGL full \& half precision.}
  \label{dgl-halfGNN-sddmmvv}
\end{figure}



\subsection{Micro-Benchmarking}
In this section we perform some micro-benchmarking to support our proposed optimization choices.
\subsubsection{Atomic vs. Non-atomic}

%compare the atomic version and non-atomic version
%(find older data, and compare with new data)\\

Atomic implementations are costly even for \emph{half-precision}, a large part of our design for \emph{SpMMve} revolved around how to mitigate or get rid of atomic instructions. This is an extremely difficult task considering how workloads are distributed around CTAs, without any latent synchronization. Furthermore, all synchronization induces overheads. But in our work, we found out that removing atomic instructions with vectored half-precision massively improves performance. Keeping everything the as it is for edge-parallel design, instead of using our vectored \textit{carry-out} design, we used atomic instructions without any vectored operation to compare how they perform. Figure ~\ref{half_atomic_vs_half2_carry_spmmve} shows the performances quite clearly across many dimensions. This is true not only for Reddit \& Ogb-product, but applies to all the other datasets also. We believe, {\halfgnn} is the first-ever such implementation, which demonstrates the performance gain using non-atomic vectorized kernels in half-precision.

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.45]{exp/exp-half-atomic-half2-carryout-spmmve-speedup.pdf} % Adjust width and height as needed
  \caption{\small Non-atomic vectored approach is much faster than half only atomic approach.}
  
  %\caption{\small Analyzing role of vectored half implementation by comparing the half-precision implementation of SpMMve with atomic and proposed non-atomic kernel, (use {\halfgnn} in legend, use speedup){ (\halfgnn} SpMMve)}
  \label{half_atomic_vs_half2_carry_spmmve}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.45]{exp/exp-half2-atomic-vs-half2-nonatomic.pdf} % Adjust width and height as needed
  \caption{\small Speedup when atomic ops removed from {\halfgnn} SpMM}
  
  
  \label{half2_atomic_vs_half2_nonatimc}
\end{figure}

%to show individually why half2 read, write matters\\


\subsubsection{\blue{Half2 is Similar to Float}}

\blue{\textbf{GNNOne-32 vs HalfGNN-64} REMOVE }

%\begin{figure*}[h!]
%  \centering
  %\includegraphics[width=0.99\textwidth,height=.12\textheight]{exp/halfgnn half vs float gcn gat gin runtime.png} % Adjust width and height as needed
  %\caption{{\halfgnn} versus {GNNOne}Training runtime for feature size = 32, 64. It can be observed runtime of HalfGNN 64 features is similar to float runtime with 32 features, demonstrating half2 vectored operation optimizations. \red{Might go in micro-benchmarking sections, redo the plot(remove)}}
  %\label{halfgnn_half_vs_float_gcn_gat_gin_runtime}
%\end{figure*} 

\blue{
We have previously mentioned that half-precision allows us to massively increase kernel throughput. In this section, we also want to compare GNN runtime with state-of-the-art {\gnnone}. This would allow us the opportunity to compare how much-vectored implementation with carryout makes a difference for complete training. From figure ~\ref{halfgnn_half_vs_float_gcn_gat_gin_runtime} some insightful observations can be made. Considering an observation between {\gnnone} feature size 32, and {\halfgnn} feature size 64, we can observe the runtime are quite close. That means we almost have the same runtime for feature size 64 using {\halfgnn}, as we get for feature size 32 for {\gnnone}. This is true for all of GCN, GAT \& GIN training. This is the empirical evidence that our half-precision kernels are integrated into the {\halfgnn} system in such a way that we have not only massively improved the throughput of individual kernel performance, but also have gained massive runtime improvements for complete GNN training. The improvements compared to {\gnnone} can be categorized loosely as: \textit{almost double}. For feature size 32, {\halfgnn} shows faster runtime than {\gnnone}. But for feature size 32, {\halfgnn} has to divide groups of features inside individual warps. This is still faster than {\gnnone}, but does not provide massive improvement for 32 features. 
}

\subsubsection{{\gnnone } vs {\halfgnn}}
Here, we showcase how {\halfgnn} kernels  perform compared to state-of-the-art {\gnnone}.

\textbf{SpMMve.} Starting with SpMMve, we compare our findings in Fig. ~\ref{exp-halfgnn-gnnone-spmmve-speedup}. To summarize, 2 distinct observations can be mentioned. One is that \red{we do not gain any speedup using {\halfgnn} \emph{SpMMve} for dim 32. (should be fine, if rerun)} Secondly, for 64 features, we get speedups an average of $1.41$ times. In some cases, we get closer to $2$ times. {\halfgnn} is different from {\gnnone} in using \emph{half2} to load, write, perform arithmetic operations, and write without atomic writes. \textit{half2}. Similar gains are observed for \emph{SpMMv}.
%{\gnnone} provides better performance for 32 features.

\red{Write a few more lines here}

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.49]{exp/exp-halfgnn-gnnone-spmmve-speedup.pdf} % Adjust width and height as needed
  \caption{\small Speedup of {\halfgnn} SpMMve compared to {\gnnone}. We gain $1.41$ times speedup on average. (\red{check G11, runs for {\halfgnn}, not yet for {\gnnone}), rerun for dim 32(rerun done)}}
  \label{exp-halfgnn-gnnone-spmmve-speedup}
\end{figure}

\textbf{SDDMM.} Here, we focus on finding out the speedup {\halfgnn} over {\gnnone} for \emph{SDDMM}. 
%In Fig. ~\ref{exp-sddmm-mul-halfgnn-vs-gnnone}, we can observe the performance gain achieved by using vectored half( \textit{half2, half4, half8}) for {\halfgnn} compared to {\gnnone}.
In SDDMM, we extend the concepts introduced by {\gnnone} for \emph{half-precision}, introducing \textit{half4, half8} rather than only \textit{half2}. \textit{half8} allows 8 numbers to be read in single memory access for individual thread and allows 8 arithmetic operations to be carried out in one go. Not only does this allow us to reduce the number of required steps during reduction for SDDMM, but also allows us to reduce the communication barrier. From Fig. ~\ref{exp-sddmm-mul-halfgnn-vs-gnnone}, we can observe that we gain on average 1.84 times the speedup. For some datasets, the number is closer to 1.5, and for others, we gain around 2 times speedup. This especially helps the GAT training. Because the attention coefficient calculation requires \emph{SDDMM} calculation.

%For this, we particularly show the performance of SDDMM of {\halfgnn} compared to {\gnnone}. One of the key reasons for choosing to use SDDMM and not SpMM for this section is that: we only used \textit{half2} for SpMM.
 %This is due to the nature of the kernel and the limitation of supported vectored type intrinsic operations being allowed till \textit{half2} only. 




\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.43]{exp/exp-sdmm-mul-halfgnn-vs-gnnone.pdf} % Adjust width and height as needed
  \caption{\small Speedup of {\halfgnn} SDMM kernel compared to {\gnnone}. On average, we gain $1.84$ times speedup.}
  \label{exp-sddmm-mul-halfgnn-vs-gnnone}
\end{figure}

\subsubsection{\textbf{Huang-float vs Huang-Half2}}.
We chose Huang et al ~\cite{huang2021understanding} as the vertex parallel work to showcase our optimizations effectiveness proposed in {\halfgnn}. Although full application of {\halfgnn} \emph{SpMM} is not applicable, we choose to apply \emph{half2} for arithmetic calculation, data load, and applied 2 stage non-atomic write process. Huang et al \emph{SpMM} performs neighbor grouping of 32 and distributes to 1 warp. Then writes it atomically. Rather than writing it atomically we store it at our \emph{carry-out buffer}, and later used pre-calculated vertex destination to write non atomically using separate kernel. The associated destination vertex is anyway saved in Huag et al. Fig. ~\ref{exp-huang-float-vs-half2}, shows the comparison of original Huang float, with Huang et al optimized with \emph{half2} techniques proposed in this work. We can see on average we get around $1.24 \times$ speedup. 

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.45]{exp/exp-hunag-float-vs-half2.pdf} % Adjust width and height as needed
  \caption{\small Huang float vs Hunag-half2 speedup. On average we gain $1.79$ times speedup.}
  \label{exp-huang-float-vs-half2}
\end{figure}

This is massive, as we are achieving this without changing any fundamental nature of Huang et al, without applying even the full range of proposed optimizations. This demonstrates the generality of our proposed optimization. 
Even though {\halfgnn} is an edge-parallel system, its design can massively improve performance for vertex-parallel systems also. \red{\td old writing}

%\textbf{half8} as never before used type, a contribution for SDDMM\\




\subsubsection{half2 vs half8 for SDDMM}
In this part, we would like to further verify how \textit{half8} would be more efficient rather than using only \textit{half2} for \emph{SDDMM}. So, rather than using \textit{half8}, we replace all of that with \textit{half2} only. This would allow us to understand the role of grouping the larger number of half-precision values better. We compare {\halfgnn} \emph{SDDMM} using \emph{half8} with only having \emph{half2}. From figure. ~\ref{exp-half8-vs-half2-sddmmvv-mul}, \textit{half8} is shown to be having speedups up to almost $3$ times. The average speedup is $1.67$ times when compared to \textit{half2} only for feature sizes $32$ and $64$. To further explain the results: when we use \textit{half8}, we reduce the number of required inter-thread communication for the reduction in \emph{SDDMM}. We previously mentioned that \emph{half8} would provide better load \& in turn less waiting time for communications to end. Nevertheless, both \emph{half8} with \emph{half2}, and \emph{half2} only {\halfgnn} \emph{SDDMM} is faster than state-of-the-art.    




%to show individually why half2 read, write matters\\


\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.44]{exp/exp-half8-vs-half2-sddmmvv-mul.pdf} % Adjust width and height as needed
  \caption{Using \emph{half8} achieves faster \emph{SDDMM} than \emph{half2} only ($1.67 \times$ faster on average)}
  %\caption{SDMMVV kernel speedup for \textit{half8} vs \textit{half2}, showing the performance gain by introducing \textit{half8} vectored type in SDDMM. On average we gain $1.67$ times speedup. Draw a line on y=1}
  \label{exp-half8-vs-half2-sddmmvv-mul}
\end{figure}

%sddmm code change for dim 32, 64

\blue{\subsubsection{Operations or Data loading the reason behind performance}}


%For SDDMMVV convert the kernels into only half operations and compare with half2 (dim=32,64)



%half2 collected: commented out all calculation from the half2-spmmve.cu (carryout version) and measured time till syncwarp(), half2 loads into shared memory.\\

%half collected: same for half dataloading, collected from only-halfspmmve.cu

%\red{\textbf{Half2 is slower.}}



%\red{previous stuff:}\\

%For our experiments we compare with CuSparse implementation, which is a standard for many frameworks, even DGL uses some kernels from CuSparse. Apart from that we also mention our numbers for these 3 kernels. 
%The datasets used for the experiments are in Table~\ref{table-dataset}. We doubled the edges, as in our experiment we treated them as undirected graphs. Hence, the edges are doubled. The graphs are downloaded from  DGL, SNAP~\cite{snap}, and the University of Florida Sparse matrix collection~\cite{sparsecollection}. Graph500 generator~\cite{graph500} is used to generate Kron-21 dataset.



%The experiment is run using Nvidia A100 GPU, which has 40GB of memory. We compared results for feature sizes 64, 128, 256, and 512. Here we only show a comparison for feature sizes 64 and 128. From Fig. 1 we can clearly see that Cusparse performances dropped during lower precision.











%So, the fastest execution is still the 32-bit version for CuSparse. CuSparse supports SpMMv. In our discussion at first, we will compare CuSparse SpMMv with our vector-type supported SpMMv.

%Let us focus on fig.2. We can clearly see from the speedups that, our proposed kernels work much faster for almost all datasets. However, in our introduction, we assumed that doubling the throughput would be possible. But it is clear that in some cases we get actually much more than that. For example, datasets such as sx\_stackoverflow, hollywood 9 we get almost 4 times the speedup. The same case for the soc-livejournal1 dataset. for datasets such as amazon, web-berkstand we get some improvements too. The fastest speedup is recorded for reddit dataset. The performances are almost similar for the 64 and 128 dimensions. Table 2 shows that vectored SpMMve implementations also have similar runtimes as SpMMv. cit-patient was also showing 2 times speedup for feature size=64, 128. We also conducted similar experiments for feature size/dims = 256, 512. It provided similar improvements.\\

%SDDMM also provided improvements while using half-precision and vector datatypes.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{comment}

\begin{table}[t]
\caption{CuSparse fastest runtime, SpMMv runtime \& SpMMve runtime (milliseconds) for feature size = 64, 128 (\red{OLD DATA})}
\label{tab:my-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|lcc}
\hline
\multicolumn{1}{|l|}{Feature size} & \textbf{dataset} & \multicolumn{1}{l}{\textbf{Vector SpMMv(16 bit)}} & \multicolumn{1}{l}{\textbf{Vector SpMMve(16 bit)}} \\ \hline
\multirow{dim = 64} & \multicolumn{1}{l|}{amazon}            & \multicolumn{1}{c|}{0.000937} & \multicolumn{1}{c|}{0.000817} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{wiki\_talk}        & \multicolumn{1}{c|}{0.001374} & \multicolumn{1}{c|}{0.001464} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{roadNet\_CA}       & \multicolumn{1}{c|}{0.001062} & \multicolumn{1}{c|}{0.001258} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{web\_berkstand}    & \multicolumn{1}{c|}{0.001022} & \multicolumn{1}{c|}{0.001317} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{as\_skitter}       & \multicolumn{1}{c|}{0.001811} & \multicolumn{1}{c|}{0.001984} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{cit\_patent}       & \multicolumn{1}{c|}{0.004274} & \multicolumn{1}{c|}{0.004606} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{sx\_stackoverflow} & \multicolumn{1}{c|}{0.004506} & \multicolumn{1}{c|}{0.004658} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{ca\_hollywood09}   & \multicolumn{1}{c|}{0.004042} & \multicolumn{1}{c|}{0.004359} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{ogb\_product}      & \multicolumn{1}{c|}{0.01115}  & \multicolumn{1}{c|}{0.011507} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{soc\_livejournal1} & \multicolumn{1}{c|}{0.007162} & \multicolumn{1}{c|}{0.007963} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{reddit}            & \multicolumn{1}{c|}{0.006842} & \multicolumn{1}{c|}{0.008450} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{orkut}             & \multicolumn{1}{c|}{0.015319} & \multicolumn{1}{c|}{0.016315} \\ \hline
\multirow{dim=128}  & \multicolumn{1}{l|}{amazon}            & \multicolumn{1}{c|}{0.001044} & \multicolumn{1}{c|}{0.001139} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{wiki\_talk}        & \multicolumn{1}{c|}{0.002472} & \multicolumn{1}{c|}{0.002642} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{roadNet\_CA}       & \multicolumn{1}{c|}{0.001916} & \multicolumn{1}{c|}{0.002278} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{web\_berkstand}    & \multicolumn{1}{c|}{0.001857} & \multicolumn{1}{c|}{0.002157} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{as\_skitter}       & \multicolumn{1}{c|}{0.003443} & \multicolumn{1}{c|}{0.003838} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{cit\_patent}       & \multicolumn{1}{c|}{0.008754} & \multicolumn{1}{c|}{0.008556} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{sx\_stackoverflow} & \multicolumn{1}{c|}{0.008196} & \multicolumn{1}{c|}{0.009123} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{ca\_hollywood09}   & \multicolumn{1}{c|}{0.007062} & \multicolumn{1}{c|}{0.008487} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{ogb\_product}      & \multicolumn{1}{c|}{0.022153} & \multicolumn{1}{c|}{0.022858} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{soc\_livejournal1} & \multicolumn{1}{c|}{0.014203} & \multicolumn{1}{c|}{0.015819} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{reddit}            & \multicolumn{1}{c|}{0.014023} & \multicolumn{1}{c|}{0.017133} \\ \cline{2-4} 
                           & \multicolumn{1}{l|}{orkut}             & \multicolumn{1}{c|}{0.030545} & \multicolumn{1}{c|}{0.032535} \\ \hline
\end{tabular}%
}

\end{table}

\end{comment}



%\begin{figure}[h!]
%  \centering
%  \includegraphics[width=0.48\textwidth,height=0.35\textheight]{figures/spmmve numbers.png} % Adjust width and height as needed
%  \caption{Performance gain while using proposed SpMMv. We compared with Cusparse 32 bit SpMMv, as half precision in Cusparse provide no improvement. Y axis is speedup (Cusparse fastest execution time/ Proposed SpMMv execution time.)}
%  \label{fig:your_label}
%\end{figure}


==> tex/others.tex <==

%\begin{figure*}[t]
%	\vspace{-5mm}
%	\centering
%	\includegraphics[scale=0.78]{figures/nnz-split.pdf}
%    \vspace{-6pt}
%    \caption{ \small Illustration of the proposed unified design for SDDMM and SpMM computation: each warp (say, 4 threads) is shown to handle 8 NZE, and 8 is feature-length for brevity. The 8 NZEs are divided among two thread groups using the proposed Symbiotic scheduling policy, where they work on 4 consecutive NZEs. Each thread fetches 4 consecutive vertex-level features from the dense matrix.}
%	\label{fig-split}
%	\vspace{-6pt}
%\end{figure*}


%\section{{\halfgnn}: Motivation \& challenges}

%GPU memory and capability have increased in recent years. But, it is still very limited compared to the requirements of training large GNNs. So, recent works have been exploring the means and ways to make sure that most of the computing resources are getting utilized, where many bottlenecks remain. For example, the training of neural networks requires a lot of state tensors to be stored, moved around, proper hardware utilization, load balancing, etc. State tensors are intermediate tensors that we need to store in each layer to carry out gradient backpropagation. 
%Datasets are generally large enough that, it is pertinent that batched solutions have to be found. This involves transferring necessary data from storage to GPU global memory \& hardware caches (shared memory, primary storage, L1/L2 cache), and the other way around for writing purposes.\\

%This leads to constraint questions, how much data be moved, how often these memory transfers must happen, while minimizing the runtime, opportunistic placements of data inside special GPU storage to reduce transfer time, and more importantly maximum utilization of threading with focus on reducing memory transfers, that too in a load balanced way. 
%Here, in our work, we believe we provide improvements to most of the existing solutions for these bottlenecks by filling gaps between GPU support and existing works and providing large-scale improvements during runtime. Furthermore, it has been mentioned before that under-utilization of GPU resources is also a big issue, and hard to overcome due to various reasons.

%Among all these, software systems must make sure provided solutions are easy enough to use, abstract the necessary things, and still provide enough maneuvering to make sure they can be part of the seamless integration of future developments of GNNs. Here, in our work, we believe we provide improvements to most of the existing solutions for these bottlenecks by filling gaps between NVIDIA hardware support and existing works, providing large-scale improvements during runtime, while keeping the necessary obligation of simplicity, necessary abstraction, and the possibility of seamless integration for future works. \\ 

%To identify these optimizations and the needs that let these optimizations be manifested, we first talk about the underlying building blocks of GNNs. 

%SpMM(Sparse matrix-matrix multiplication), and SDDMM(Sampled dense-dense matrix multiplication) are the 2 key sparse kernels that constitute all that there is to these software systems targeting GNNs. Another important factor that lets researchers separate away these 2 from normal GeMM (General Matrix Multiplication) is the unstructured sparsity factor lying with every call of SpMM and SDDMM in the GNNs. 
%This sparsity originates in the unstructured topology that lies inherent to graph datasets. This requires studying data transfer patterns that reduce the number of transfers in general. Here, we notice a gap between GPU hardware systems and existing software systems (CUDA kernels). To be precise, GPU hardware supports lower precision (16 bits, relevant for this work). But implementations, research works, and frameworks either do not utilize this at all for GNN training, when does so, do a poor job at it. 

%We propose 16-bit based SpMM, SDDMM kernels that can produce trained GNNs that perform well, with multiple magnitudes faster runtime. 
%These existing issues can be identified at a glance, SpMM calls without edge reductions being plotted in Fig 1. We see that CuSPARSE half precision is very slow compared to its 32-bit counterpart, let alone providing improvements, which is the standard go-to library for any sparsity-related computations for GNN. The theoretically faster throughput is missing even in standalone calls. 2nd question that needs to be answered if training in 16 bits is enough. Recent works ~\cite{micikevicius2017mixed, gupta2015deep, hubara2018quantized, hubara2016binarized} have shown to varying lengths that lower precision is enough. We go into further detail about the intricacies involved that have been explored and our solution in later parts. Our work is working fine across robust measurements and maintaining model effectiveness.\\


%Our evaluation shows incorporating these techniques makes SpMM and SDDMM to run almost twice as fast (compared to 32 bit implementations of the same SpMM and SDDMM). Compared to cusparse, we achieve multiple magnitudes of faster runtime. %Another important factor is DGL uses mostly their own implementations for GNN training, where for some they utilize cusparse. 
%Our implementations of SpMM and SDDMM, outperform CuSPARSE and in general, we achieve faster runtime. We also made sure warp utilization is maximized and the workload is balanced across SMs. Lastly, for implementing our experiments and optimized kernels, we choose GraphPy, a framework-neutral API, this allows reduced implementational overhead and allows users to focus on Cuda Kernels only. \\



% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.48\textwidth,height=0.23\textheight]{figures/Cusparse 64 vs 128.png} % Adjust width and height as needed
%   \caption{SpMM kernel comparison in speedup (32 bit runtime/16-bit runtime). half-precision performs slower.}
%   \label{fig:your_label}
% \end{figure}



%\begin{figure}[h!]
%  \centering
  %\includegraphics[width=0.48\textwidth,height=0.12\textheight]{figures/gnn single vs half runtime.png} % Adjust width and height as needed
  %\caption{GCN, GAT, GIN runtime in single precision \& half precision.}
  %\label{fig:your_label}
%\end{figure}



%\subsection{{\halfgnn}: Overview } 

%The number of threads that can be launched is GPU-specific and limited. What designed solutions are looking for: is to perform the maximum number of kernel computations, with the maximum possible thread launch. This often relies on how the kernels are being designed. Data load being the costliest operation, it is directly dependent upon the maximum number of kernel computations/launches that are possible, in any design. Only necessary data is performed for the kernels, and this data is kept on GPU memory to take advantage of its fast access. This leads to peak possible performance for that designed solution, considering whatever approach the kernel design follows(vertex level, feature level, or other kind of parallelism), even though many threads launched do not often reach the peak hardware limit. So, if we can increase the possible number of computations in the same number of clock cycles, we can achieve better utilization of fast dedicated GPU memories. This is where the optimization opportunity lies, GPU memory and thread parallelism both are underutilized. We propose to massive improve this.\\

%Considering 16 bits for all tensor operations in forward and backward during training, what we will show that we can use \textit{half2} datatype for all computations. Simply, put allowing one to do 2 arithmetic operations in 1 vector operation instead of 1 calculation. Then each thread can achieve twice the number of computations using the same clock cycles (later explored in detail). This allows us to also increase the number of possible thread launches, increasing the utilization of parallelism offered by GPU hardware ( or write: getting closer to the absolute hardware limit). Because following our design we can double the per-kernel computation, keeping the memory requirement for each kernel the same. Later sections will further explore the details of how this is achieved. As pointed out before: data loading is done based on requirement by kernel launches. As, we can achieve twice the kernel launch that that same time, this also allows us to perform twice the data load, achieving a 100\% increase in memory utilization and thread utilization. This is one key contribution, as this directly removes the under\-utilization problem and, at the same time allows for doubling the parallel data, pushing the existing state-of-the-art very far.\\

%(remove)write about data\-loading done in kernels (later or now)\\

%As mentioned previously, dataloading  is done based on how much computations are being carried out by each kernel, the number of kernels launched, \& kernel design.\\

%One of the key design aspects we need to look at is the kind of parallelism introduced and the resultant work\-load distribution resulting from it. Assigning equal work\-load does not only make overall computations faster, but it also allows for faster data load in the coalesced manner by the warps to maximize overall performance.  
%Most works design their kernels either in a vertex-parallel or feature-parallel manner. Some of the examples are: (from COOGNN paper) DGL assigning each computing unit a fixed number of vertices. Similarly, GE-SpMM ~\cite{gespmmsc2020}, and FeatGraph ~\cite{featgraphsc20} allocate equal compute units to process each row. The problem with this approach is vertices do not have an equal number of neighbors, resulting in an uneven distribution of work. GNNAdvisor ~\cite{wang2021gnnadvisor} and Huang et al ~\cite{huang2021understanding} use the neighbor grouping to handle the workload imbalance. They split a row into several neighbor groups if the degree is greater than a threshold, usually set as 32. But this requires additional computation and metadata, additionally, there is no fixed choice of the neighbor grouping parameter, and each can result in very different outcomes. Then each group is assigned to different warps and parallelism is carried out in a feature-level manner. This leads to the under-utilization of warps. Some threads remain idle in these solutions. For feature parallel solutions, if the feature-length is less than 32, threads will remain idle. \\

%Rather than these approaches, our design follows edge-level parallelism (cite COOGNN). This approach ensures the aforementioned shortcomings are removed completely. The approach is to have a fixed number of nonzero edges to be assigned to each warp, and each thread working on 2 features. How to assign each thread to work on 2 feature is elaborated in later sections. Edge-level parallelism allows equal distribution of work distribution at the same time ensures all threads are working in the warp. The problem that feature-level parallelism had of idle threads for feature length less than 32, is handled through further grouping the nonzero edge groups and distributing them equally among the threads.% We will clarify with a later example(necessary/unnecessary).


==> tex/related.tex <==
\section{Related works} \label{sec.related}

%(change the talk to different problems being addressed, rather than only GPU hardware research gap, eliminate the last paragraph totally, irrelevant, commented out line 14)\\

GNNs have been explored mostly for float data-type~\cite{chen2020fusegnn, pytorchg2019, fu2022tlpgnn, featgraphsc20, schlichtkrull2018modeling, liang2020engn, dgl2019, wang2021gnnadvisor, wu2021seastar, yan2020hygcn, zhang2021boostgcn, gaan2018, ye2023sparsetir}.  
%liu2015enterprise, wang2015gunrock
%Recent developments in GPU hardware provides tensor core. These cores are very useful in faster implementation of dense matrix multiplications. 
Wang et al~\cite{wang2023tc} used tensor core to increase computation efficiency for the sparse kernel. 
%possible computations when sparsity is involved. The problems is that these tensor cores are designed in such a way that it takes tiles from 2 participating matrices and have specific hardware that implements dense tiled matrix multiplications. 
But for graph neural networks, the data has unstructured sparsity, and hence tensor core does not help. 
%it does not help as we are dealing with sparse topology in graph neural networks, and matrices are mostly sparse. 
Due to this, prior works~\cite{Graphpy} have shown that TC-GNN performs even slower than float-based GNNs.

%So, in our work there is no possibility of using this computing unit to improve performance. All of our solution work on GPU core.


Most graph datasets are sparse, this poses different kinds of challenges for training GNN. Most common graph neural networks are GCN ~\cite{kipf2016semi}, GAT~\cite{gat18iclr}, GraphSage~\cite{graphsage17} and others~\cite{zheng2021dgcn, gaan2018}. 
2 constituting operation of any GNN model are gather-scatter operation(aggregation)~\cite{gonzalez2012powergraph, kipf2016semi, gat18iclr}, and update phase. Although part of these operations is very similar to Linear layers of NN, it has great differences in terms of required computation to be carried out. The main difference is sparsity. 
There exists a large portion of unnecessary computations that are irrelevant and is not feasible to be carried out in an efficient manner in current hardware/GPU support, not to mention lack of efficiency. As these computations are different from highly optimized dense matrix-dense matrix multiplications, they have to be optimized using different techniques.  

This aggregation and update rely on matrix multiplication kernels that carry out these operations in fastest possible manner. Although underlying computation is simply matrix-matrix multiplication, the optimization opportunities and computation efficiencies largely rely on what kind of matrices are being multiplied. These are ideally sparse matrix dense matrix multiplications, and dense matrix dense matrix multiplications. Multiplication between 2 dense matrices is studied and quite well suited for efficient computing. CuBLAS ~\cite{nvidiacublas} is the library that is often used for these dense and highly optimized matrix multiplications (General Matrix\-Matrix Multiplication: GeMM). The problem is that in GNN computations are not dense, and these highly optimized libraries do not exist for sparse matrices. CuSPARSE ~\cite{nvidiacusparse} is the most commonly used library that is leveraged by frameworks such as DGL ~\cite{dgl2019}, pytorch geometric~\cite{fey2019fast}. Though cuSPARSE supports optimized kernels for sparse matrix-dense matrix (SpMM) multiplications), it is not as optimized as dense ones~\cite{wang2023tc}. This is due to the fact that hardware can not be optimized for unstructured sparsity, and thus kernel designs are the only thing that can be explored for optimization. Apart form that cuSPARSE only uses CUDA cores and does not support any recent optimizations supported by TCUs. The reason for that simply is large sparsity and this sparsity is unstructured. So, all the optimizations that can be achieved need to be implemented using CUDA cores only, and with mostly through kernel design, and resource utilization. So, possible optimizations are not as straight forward as for GeMM. another important observation that is well-known in the underutilization of resources. As pointed out by ~\cite{wang2023tc}, it is often the case that the available memory in GPU is underutilized.  Some of the key problems that arises with the hardware constraints are limited GPU memory, limited thread execution, handling concurrency, handling read/write in an efficient manner, etc. We will explore some of these limitations, and bottlenecks in more detail in later sections.  \\

Furthermore, we want to talk about two very specific advancements that would allow for a lot of optimizations that are proposed in this paper with the goal of pushing the existing state of the art. These are: (i) GNN with lower bit precision, and (ii) introduction of vector types. Many works such as ~\cite{micikevicius2017mixed, gupta2015deep, hubara2018quantized, hubara2016binarized} have shown it is possible to achieve the same results with a smaller number of bits. Courbariaux et al. at ~\cite{courbariaux2015binaryconnect} have shownh even using -1 and 1 as training weights is often enough to achieve good results, Hubara et al.~\cite{hubara2016binarized} also used binary activation to achieve good performances. Hubara et al ~\cite{hubara2018quantized} have also quantized the weights and explored what are the outcomes. But these are often not shown in diverse kind of datasets. Among all these varied lower precision implementations, Micikevicius et al. ~\cite{micikevicius2017mixed} have shown that it is entirely possible to carryout the bulk of the computation for deep learning in lower precision 16 bits) with all kind of models and with no compromise in any kind of performance. This improves memory requirements, but this alone does not necessarily improve the overall parallelism that can be achieved in general for kernels required for GNN training. 
This is where the second concept of grouping 16 bit numbers to vector types~\cite{ho2017exploiting} and vector operation can help out a lot. To simply put, allowing multiple lower precision numbers to be grouped together (group of 2) and having single thread to carry out computing operation on the group in single clock cycle at a time, rather than carrying out operation between only 2 operands constituting 2 floating point numbers. This ideally would be able to double the throughput per thread, but this can not be incorporated in existing solutions so easily. We propose many optimizations in kernel designs that combines both of these advancements, and produce new highly optimized kernels that achieves at least 2 times the speed up from existing state of the art, at the same time massively improving many of the existing bottlenecks. \\




\red{(DONE) APNN\_TC, EGGMM\_TC, tensor Core-Based GPU Kernels }

Feng et al. ~\cite{feng2021apnn} bridged the gap between, need for different precision required for layered DNN with limited precision supports in recent hardware architectures with tensor cores. The support provided by new hardware precision supports were not enough, i.e limited precision with limited mathematical operation support in tesor cores. This required engineering emulation designs that supported diverse precision operations to be mapped onto the tensor cores. This was designed for Ampere architecture. Introduced emulation design for varied precision, improving efficiency in DNN layers through kernel fusion, and faster data movements allowed for great improvements in speed. This is one of the first works that full take advantage of the available tensor cores.\\


Similar but slightly different work such as EGMM-TC ~\cite{feng2021egemm} provides emulation for GEMM in extended precision to take advantage of the tensor cores fast computing capability. One of the key challenges was to manage half input for tensor core and not loose precision for precision heavy applications. This was done by creating a lightweight and novel emulator for extended precision. Previous works provided performance improvements in terms of speed using half precision, but this reduced accuracy in precision. Along with the emulation algorithm, ~\cite{feng2021egemm} also provides new optimization for tensor mapping to efficiently map workload to tensor cores.\\

None of these works are applicable in the problem space we are working on, that is unstructured sparsity. To emulate and to organize unstructured sparse data for tensors input would incur a large overhead. As the 2 previously mentioned work had to deal with that even for GEMM, which does not suffer from sparsity at all. Thus there is no feasible use for current characteristics of tensor core, under the problem space that we are working on. 

\begin{comment}
\section{Related Work} \label{sec.related}


old stuff:\\
GNN are very important are in Deep learning with ever growing applications. Recent works such as ~\cite{gupta2015deep} have shown 16 bit precision for CNN works fine for MNIST and CIFAR-10 dataset. Some works even used binary weights and binary activations to achieve good results ~\cite{hubara2016binarized, courbariaux2015binaryconnect}. Furthermore, quantizing, rather than using binary weights was also fine for training~\cite{hubara2018quantized}, and was somewhat similar to using floating points(32 bits). Micikevicius et al. ~\cite{hubara2018quantized} have shown the steps to use half precision as part of training and introduced 3 key steps so that diverse models on diverse datasets can be trained. We followed the same approach and optimized kernel implementations in half precision. These are the kernels that would be computing gradients in 16 bits, which is recommended by the paper.So, speedups achieved by us would work.

There exists many systems. Optimizations are important in these and a lot of system optimizations have been proposed ~\cite{wang2023tc,fu2022tlpgnn,wang2021flexgraph,hu2021efficient,jangda2021accelerating, liang2020engn, zhang2021boostgcn, kim2022analyzing, yan2020hygcn,ye2023sparsetir}. As we have discussed in our background studies that SpMMv, SpMMve and SDDMM are the main kernels that are used for state tensor operations, it is important to optimize them as much as possible.
%\subsection{SDDMM and SpMM Related Works } \label{sec.balancing.analysis}
In this study we compared with CuSparse SpMMv variant. We focused on 32 bit and half precisions also.

\noindent \textbf{SDDMM.}
One of the most used frameworks in DGL and it also uses SpMM from CuSparse. So, comparing with CuSparse also gives good comparison of these kernels being used by DGL for GNN training. Other works such as ~\cite{gale2020sparse,featgraphsc20} uses vertex-parallel variants. These 2 works lacks workload imbalancing and also does not support caching. A different variant such as Sputnik~\cite{gale2020sparse} does not reuse vertex-level features for row indices. 


%\noindent \textbf{Custom Storage Format}.
\noindent \textbf{SpMM.}
GE-SpMM~\cite{gespmmsc2020}, FeatGraph~\cite{featgraphsc20}, TLPGNN~\cite{fu2022tlpgnn} follow vertex-centric SpMM. Vertex-centric approaches suffer from workload imbalance, and it is the same case for these papers. Edge-centric SpMM of
Yang et al.~\cite{yang2018design} performs even slower than vanilla vertex-parallel SpMM as reported by itself. 

Some of the works such as 
GNNAdvisor~\cite{wang2021gnnadvisor}, Huang et al~\cite{huang2021understanding}, 
Sputnik~\cite{gale2020sparse}, ASpt~\cite{hong2019adaptive} proposed a \textbf{custom storage format} and preprocessing to provide workload balancing in SpMM. In our work we do not need these metadata or preprocessing at all.
GNNAdvisor~\cite{wang2021gnnadvisor}, Huang et al~\cite{huang2021understanding} divides each row into several groups 32 non-zero columns.

Although this is an interesting approach, the problem is that rows are hardly multiples of 32. So, load balancing is not perfect, and this work still have problems of workload imbalance.

 Prior works~\cite{yang2018design,featgraphsc20,gespmmsc2020,huang2021understanding,wang2021gnnadvisor} uses Vanilla feature-parallel methods. They assign one thread to fetch one feature. Then memory barriers have to be used and it impacts performances.
 
 \noindent \textbf{Kernel Fusion for GNN} Kernel fushion is a very common technique to improve performance. Works such as ~\cite{wu2021seastar,chen2020fusegnn,zhang2022understanding} fuse GPU kernels using vertex-parallel approach. Althought this works for SpMM, but this approach does not help SDDMM. SDDMM are naturally edge-parallel. 

\noindent 
\textbf{Graph Processing.} 
Some works rely on binning~\cite{liu2015enterprise,wang2016gunrock} for workload imbalance. They distribute to different bins by using preprocessing. This is an additional step that we do not need for our work.


%Additionally, many SpMM works use the \textit{feature-parallel} method, which is explained later in this sub-section. However, they have not succeeded completely. 


\end{comment}

% \noindent 
% %$\bullet$ 
% \textbf{Vertex-Level Parallelism.} 
% When the column of non-zero elements has a scalar feature, gSpMM becomes gSpMV and is shown in Algorithm~\ref{algo-pr}.
% The for loop here is a candidate for vertex-level parallelism, where a thread or a warp is responsible for all computation involving one row. 
% This leads to workload imbalance as some rows have more non-zero elements than others, which we focus on in this work. 

%Rather many real-world graphs have a large variation  count, where a few vertices have a really large number of neighbors.
%To demonstrate this, we plot the degree distribution of the Reddit dataset, which is a popular data set used in GNN.\red{not sure}. 
%Edge-level parallelism is defined when each thread works on an equal count of edges, e.g. by using the COO format. However, prior works have not achieved better SpMV results~\cite{bell2009implementing}, which we explore in this paper.
%may help alleviate the problem, but it requires two changes: materializing the per-edge messages during scatter, and  using the costly atomic instructions while gathering messages to update the vertex-level output.


% %While analyzing workload imbalance, 
% These two techniques have inherent workload imbalance in two aspects of GPU.
% (a) Vertex-parallel sparse kernel introduces \textit{inter-warp} workload imbalance as a few warps are assigned more work than other warps, and hence less loaded warps may remain idle while the more loaded warps continue execution.
% In (b) Feature-parallel sparse kernel introduces \textit{intra-warp} workload imbalance as it is possible that some of the 32 threads of the warp may not have works to perform due to feature-length being not a multiple of 32, which is a very common case in GNN. Hence those threads remain idle, and we lose performance. 

%We would also like to point out that the workload balancing alone is not sufficient if it cannot take advantage of the performance-critical GPU attribute. 

%Many GNN works feature-level parallelism as a baseline implementation on top of which they proposed various inter-warp workload balancing techniques that we discuss next.

% \subsection{Hypothesis and Analysis}
% In this sub-section, we start with our hypothesis of what leads to workload imbalance. Based on the hypothesis, we propose a new solution and explain how our work solves this workload imbalance problem. However, before we fully delve into the complexities of the solution, we discuss whether the proposed idea can be beneficial or not by relying on the upper bound of the performance.



%\noindent  $\bullet$ \textbf{Vertex-Parallel.}
%DGL has its own implementation of some SpMM kernels using vertex-parallel method on CSR/CSC format, as Cusparse does not provide all the implementations, specifically when the reduction operation is not \textit{sum}. For SDDMM, it relies on its own SDDMM  using the COO format in edge-parallel way to achieve workload balance. While DGL motivated our work to use COO for every sparse kernel, it has no data reuse. Hence, proving our earlier point (\cref{sec.intro}) that workload balancing alone is not sufficient. 
%\textit{one size fits all} solution, i.e. allocate equal compute units to process the N(v) of each vertex irrespective of the size of N(v). 


%A technique from graph analytics works is
%(2) \textbf{The rigid nature of thread assignment}  to each vertex irrespective of its neighborhood size does not help in alleviating the problem. A few prior graph solutions~\cite{liu2015enterprise} do try to solve this problem 

%Hence, if a row has 33--64 non-zero elements, it will be broken into two groups, and hence will be allocated two warps.
%and hence rows will have the last group less than 32 non-zero columns as well as rows that have row-length than 32. They all still get one warp to process them, thereby creating imbalance. 
%Sputnik's row swizzling is based on the internal knowledge of the warp scheduler that produces additional array of row ID in decreasing row-length for SpMM. However, it follows a different strategy for SDDMM.
%ASpt~\cite{hong2019adaptive} custom format is different for SpMM and SDDMM, and hence it is a system with two custom formats.


%The offset array is then modified that contains an entry for the same vertex two times and also stores the vertex ID explicitly.
%Both works use the warp-based task assignment, i.e., it assigns one warp to one neighbor group, and the warp uses threads to perform feature-level parallelism.

%and uses each thread within the warp to aggregate one dimension of the node embedding. 
%By splitting the large neighborhood into multiple neighbor groups, it hopes to achieve workload balancing. 
%Another technique is to divide N(v) a vertex and allocate a GPU warp to each part. This is practiced by GNNAdvisor~\cite{GNNAdvisor}, and by Huang et al~\cite{huang2021understanding}. Apart from the fact that they use atomic instruction in this case to achieve vertex-level computation, it 
% Sputnik~\cite{gale2020sparse} also proposed a custom storage format through a 
% row-swizzling pre-processing step that produces another array containing rowID in a specific order to take advantage of how the warps are scheduled in GPUs so that a warp handling the row with the largest degree gets scheduled earlier. \td check if it followed the same approach for SDDMM.


%the where each thread processes the same non-zero element in feature-level parallelism way before it goes to the next non-zero element. 
%Hence, when feature-length is not a multiple of 32, several threads of the warp remain idle, leading to another form of workload imbalance within a warp, or compromises on their original design.Indeed, we have seen multiple cases where feature-length is not necessarily a multiple of 32. In GCN and GAT, the feature-length of the last layer depends on the number of predication classes, such as 6 in Citeseer. 
%Moreover, in the original GCN and GAT implementation, 16 is the intermediate feature-length.

%Despite the proposal of a custom storage format and feature-parallelism, none of the prior solutions are flexible enough to completely eliminate workload imbalance as they are merely an extension of the vertex-parallel method, except for a few edge-parallel SDDMM of DGL, which lacks data reuse.  


% %\subsection{SDDMM Related Works}
% Not many optimizations have been proposed for SDDMM. 
% %We show that the 2-stage data-load improves data-reuse hugely.
% ASpt~\cite{hong2019adaptive} also proposes custom storage through pre-processing. But their pre-processing is different for SpMM and SDDMM, and hence it is a system with two formats. Sputnik uses vertex-parallel approach for SpMM and SDDMM both.

%{SpMV and Graph Processing Related Works}
%We now discuss gSpMV and graph analytics systems, which though not the focus of this paper, present us with some relevant workload-balancing techniques. These works  consider only scalar features.

%Bell et al~\cite{bell2009implementing} proposed \textit{row splitting} in GPU, where every row is processed by usually by one warp, and hence offered no workload balancing.
%Vertex-parallel sparse kernel introduces inter-warp workload imbalance as a few warps are assigned more work than other warps, and hence less loaded warps may remain idle while the more loaded warps continue execution.

%Some variant do exist though.  also uses a variant of the binning technique. 
%assigning either one thread, warp, or block to process N(v) of one vertex. 
%However, it slightly differs for the rows whose degree is even larger: it separates edges into equal-length chunks and assigns each chunk to one CTA. %In that way, the frontier with large neighbor list size splits its neighbor list into multiple chunks. To find the starting and ending indices of these multiple chunks, Gunrock uses an online search method.


%\textit{Though vertex-parallel method does not achieve any workload balancing; row binning, despite proposing a custom storage format, is still not flexible enough to solve the workload balance completely, as it is merely an extension of vertex-parallel methods.}

%Binning solutions that we discussed in \cref{sec.related}  allocates either one thread, one warp or one thread-block per N(v), etc. This solution is like \textit{three size fits all} approach. Due to such \textit{rigid thread assignments},  one cannot allocate a variable number of threads, warps, or thread-blocks to process N(v) of different vertices. Hence, such solutions cannot  eliminate workload imbalance completely.
 
%uses a hybrid technique to handle the workload imbalance.If the size of the frontier’s neighbor list is small, Gunrock uses a fine-grained strategy, assigning one thread to process N(v) of each vertex. 
%Therefore, each thread handles the workload of the assigned frontier’s  neighbor list.
%Otherwise, Gunrock uses a threshold to decide whether choose a node-based coarse-grained strategy or an edge-based coarse-grained strategy. If the number of frontiers is smaller than the threshold, Gunrock adopts the node-based coarse-grained strategy. Gunrock first labels the frontiers into three categories based on it’s neighbor list size (large, medium, and small). Gunrock provides the processing strategy for each label category individually: For the frontier with a large neighbor list, all threads in the block will be used together to process its neighbor list. For the frontier with a medium neighbor list size, each warp will handle one frontier. For the frontier with the small neighbor list, each thread will handle one frontier.  To be more specific, When the kernel process the frontiers, within each block, Gunrock will first pick the frontier with the largest neighbor list size as the winner node and check its label. If its label is large, Gunrock uses the corresponding techniques to process it and then picks a new winner from the remaining frontier and repeats this procedure. However, this procedure will stop when finished processing all frontiers with a large label. After that, Gunrock does not pick any winner nodes. Instead, it uses the strategy above directly to process the remaining frontiers. On the other hand, If the number of frontiers is larger than the threshold, Gunrock uses the edge-based coarse-grained strategy. 



%minimize the number of items  
%Secondly, we use the thread-local variables to store the partially reduced results, and use warp intrinsic to do the final reduction. We believe the change in approach plays an important factor that is the main reason for the better performance improvement.
% \textbf {\textcolor{red}{optimization works for spmv}}
% \textbf {\textcolor{red}{spmv has different optimization opportunities than spmm}}

% Dalton et al~\cite{dalton2015optimizing} proposed to split the non-zero elements of the sparse matrix equally among CTAs using a pre-processing phase that generates new metadata containing starting and ending row ID and column ID for each CTA. Within a CTA, each thread gets equal work using the \textit{strided-spmv} method which again cannot allow thread-local reduction. Rather they write each dot product to shared memory as a pre-requisite to perform the reduction.

% Merrill et al~\cite{merrill2016merge} include the number of writes (CSR rows) along with the count of non-zero elements when dividing the work among CTAs, otherwise, it is very similar to a non-zero split method. A pre-processing step using merge-path algorithm~\cite{odeh2012merge} generates new metadata for each CTA. It uses the \textit{blocked-spmv} method to divide the work between threads of a CTA, however, it uses an online invocation to merge algorithm to generate the work for each thread and finds the row ID for non-zero elements. This allows thread-local reduction before it performs some inter-thread communication.

%is transposed from strided to blocked order using shared memory and a CTA-wide segmented scan is performed. Hence, no online search is needed with each CTA.
%Some rows containing a large list of non-zero elements will be split into multiple CTAs. In that case, merge-based SpMV uses the fix-up kernel. 
%to reduce the aggregated value, including spawning another kernel to do the same for N(v) which is split across CTAs.


%but the materializes each dot product to the shared memory to perform the reduction due to the usage of the strided method. The performance is very sensitive to how many dot products are materialized, and where are they materialized. We did not follow this method at all. 

%Unlike previous works try to parallel based on the rows of CSR, or simply parallel based on the number of non-zero elements in CSR. Merrill treats both the number of CSR rows and the number of non-zero elements as the total workload and divides the total workload by the number of threads and assigns each division result to one thread. Therefore, Merrill maintains the workload balance. 
%To be more specific, each thread-blocks are allocated a similar amount of non-zero elements, whose starting and ending row ID and column ID need to be searched, which is achieved using merging algorithm~\cite{odeh2012merge} as a pre-processing step. 
%After that, Merrill splits the merge path to the thread-blocks and each thread-block will get a path including a vertical or horizontal subpath. 

%that does not allow coalesced memory access of column ID, and edge feature. 

%despite dividing the work equally among threads.
%On the other hand, the advantage is that each thread can do a local reduction without using shared memory for allocated non-zero elements and only one item per thread is needed to be reduced among warp threads, compared to reducing all the dot products in Dalton et. al.

% The solution achieves perfect workload balance at the cost of materializing all dot products. We implemented this approach and were able to see that the materialization cost in gSpMM is huge due to vector features.
% Since each thread works on different chunks of non-zero elements, the threads of a warp do not get a chance to form a coalesced memory access for non-zero elements and edge features. 

%--------------------
% \noindent \textbf{gSPMV Design Trade-Off that is avoided by gSPMM.}
% Dalton et al and Merrill et al present an important design trade-off in the case of SpMV using CSR, \textit{which unfortunately has not been evaluated}. Dalton et al (strided-spmv) coalesce memory access for non-zero elements and edge features at the cost of introducing huge inter-thread communication for the reduction of each dot product, which was achieved using materializing them in the shared memory. While Merrill et al (blocked-spmv) trade-off coalesced memory access to introduce thread-local reduction so that only one item per thread requires inter-thread reduction. 
% %Interestingly, these two design choices have not been evaluated.

% However, we argue that {\name} avoids this trade-off for gSpMM, and adopts the strengths of both designs due to the caching. As discussed previously, caching coalesces memory access of non-zero elements and edge features irrespective of whether {\name} uses the strided or blocked method.
% %but it also enables the implementation of the blocked method that can do a thread-local reduction.
% Further when the feature-length is a multiple of 32, strided and blocked converge to the same implementation. It should be noted that caching has no benefit in gSpMV where the feature-length is one, as the job of caching is to avoid the repeated fetch of non-zero elements and edge features by different threads that operate in a feature-parallel way in gSpMM. 


% \noindent \textbf{Summary.} 
% The current gSpMM works are still \text{vertex-centric}, thereby indirectly giving precedence to reduction work instead of the data load phase. Hence, these works cannot achieve good data load balancing. 
% In contrast, our work treats data loading as the lead phase and designs the reduction based on the data load. 
% Our work is related to a line of gSpMV work, called \textit{non-zero spliting} or its variants~\cite{dalton2015optimizing,merrill2016merge,hola2017ipdps}, which are discussed in \cref{sec.related}.





%FeatGraph~\cite{featgraphsc20},Huang et. al., GE-SpMM, and GNNAdvisor  have all used feature-level parallelism~\cite{yang2018design}. It implies handling different feature dimensions by separate threads of the warp, and thus fetching the features results in coalesced memory access.However, 
%{these works} have huge intra-warp imbalances when the feature-length is not a multiple of 32. 


%Merge-based solutions~\cite{merrill2016merge} does provide equal work to each thread, however workload balancing itself is not sufficient to achieve good performance as absence of coalesced data access does not allow it to perform better as we identified earlier. Since, its pre-processing step generates additional metadata for each block and its threads, and hence threads do not work on consecutive non-zero elements.


%Though the COO format allows us to prototype both approaches without any pre-processing or any complexities.  Also, there is only one feature in the SpMV, so overall one dot-product involves bringing column ID, vertex feature, and edge feature, but in our approach, it will additionally bring row ID as well. Hence, overall we are likely to do 25\% additional data load and do not expect to perform better than these two in our current implementation.

%It should also be noted that the natural extension of both approaches for gSpMM is not {\name}. Dalton et al use a strided method of workload division, hence they can easily borrow feature-level parallelism and thread-group concept, but will suffer from the issues mentioned due to the strided method including excessive writes to shared memory for each dot product.
%Rather, even Dalton et al uses shared memory to do reduction, and hence it will end up using a huge amount of memory. 
%On the other hand, 
% It should also be noted that the natural extension of Merrill et al is not {\name} unless they borrow the idea proposed by {\name}, and have to drop the reliance on the CUB library for reduction. 
% They perform blocked access, where the work is allocated by an online search step.
% %Hence, it will not be able to borrow feature-level parallelism without changing the pre-processing step. and unlikely to use our thread-group. 
% Thus, each thread is likely to process all the features of non-zero elements assigned to it and hence cannot incorporate feature-level parallelism and thread-group without significant changes to its design. It will also not be able to coalesce memory access for non-zero elements and edge features.
%We argue that when CSR format is used to generate 


%which is managed in the GPU-shared memory. 
%For the vertical subpath, the thread will perform the matrix-vector dot operation. For the horizontal subpath, the thread will perform the aggregation to reduce the dot operation results to output. 
